Unitriangularity of decomposition matrices of the unipotent ${\ell}$-blocks for simple adjoint exceptional groups

In 2020, Brunat-Dudas-Taylor showed that the decomposition matrix of unipotent ${\ell}$-blocks of a nite reductive group in good characteristic has unitriangular shape, under some conditions on the prime ${\ell}$, in particular ${\ell}$ being good. We extend this result to ${\ell}$ bad by adapting their proof to include the ${\ell}$-special classes dened by Chaneb.

==> casesleft__1_.tex <==
We now have the tools to check the conditions in Proposition \ref{prop_excellent} for the two  $\ell$-special unipotent conjugacy classes of $\G$ for which we can not apply Corollary \ref{cor_genial}.
\begin{lem}
The unipotent classes in Proposition \ref{prop_casesleft} satisfy the conditions of Proposition \ref{prop_excellent}. 
\end{lem}
It suffices to show the existence of an admissible covering and the conditions in Proposition \ref{prop_DecKawExc}.\\

For the rest of this section, we assume that $\G$ is simple of type $E_8$. For each simple root $\beta \in \Delta$, we set $\omega_\beta$ the fundamental dominant coweight corresponding to $\beta$. We fix a bijection $\alpha$ from the semisimple elements of $\T^*$ to the Kummer local systems on $\T$. For $t \in \T^*$, by \cite[Prop.~4.4]{acharLocalisationFaisceauxCaracteres2010}, we have \[W_\Ll \cong W_{C_{\G^*}(t)}(\T^*).\]


\subsection{The unipotent conjugacy class $E_6(a_3) + A_1$ when $\ell = 3$} 
We fix the setting in the case where the $F$-stable unipotent class is $\Cc = E_6(a_3) + A_1$. We choose $t \in \T^*$ such that $C_{\G^*}(t)$ is of type $E_6 \times A_2$ and $v \in C_{\G^*}(t)$ lies in the unipotent class $A_2, 111$ of $E_6 \times A_2$. 

\subsubsection{Admissible covering}
We follow \cite[$\S$ 10.2]{brunatUnitriangularShapeDecomposition2020}. We can choose $s = \omega_{\alpha_1}(1/2)$ and $u_\Cc \in C_\G^\circ(s)$ $F$-fixed. In that case $C_\G(s)$ is of type $D_8$. We set $\H \defeq C_\G({s})$. Thanks to Algorithm 5.2 in \cite{brunatUnitriangularShapeDecomposition2020}, since only one unipotent class of $\H$ fuses into $\Cc$, we know that $u_\Cc$ lies in the unipotent class $6631$ of $\H$ which fuses into $E_6(a_3) + A_1$. 
The group  $A \defeq \langle {s} \rangle$ can be chosen as an admissible covering of $A_\G(u_\Cc)$ for a fixed cocharacter.  Observe that $$A \cong A_\G(u_\Cc) \cong \Omega_{C_{\G^*(t)},(v)_{C_{\G^*}(t)}}$$ and if $\ell = 3$, then $ A \cong \Omega^\ell_{\G,\Cc}.$

We are left to check the last condition of Proposition \ref{prop_DecKawExc}.
\subsubsection{Character sheaves} 
We fix $\Ll \defeq \alpha(t) \in \mathcal{S}(\T)$. We now consider a principal series character sheaf of $\G$ coming from $\Ll$ with unipotent support $E_6(a_3) + A_1$. Thanks to Lusztig's map ( \cite[Thm.~10.7]{lusztigUnipotentSupportIrreducible1992}), in CHEVIE notation, we choose the one corresponding to the character $\phi_{30,15},111$ of $W_\Ll$. Observe that $\Aa \defeq \Aa^\Ll_{\phi_{30,15},111}$ is $F$-stable.\\
Using CHEVIE, we compute that $W^{\H}\backslash W /W_{\Ll} = \{1,g\}$ for some $g \in W$. The groups $W^{\H} \cap W_{\Ll}$ and $W^{\H^g} \cap W_{\Ll} $ are both Weyl groups. Therefore $\chi^{s}$ and $\chi^{s^g}$ are trivial, by Lemma \ref{lem_valchiz}. We can thus use the Mackey formula to simplify Proposition \ref{prop_formula}. 
In that case, it becomes for any $E \in \irr(W_\Ll)$
\[s^*((\Aa_E)_{\vert s \H_{uni}})[-\dim(\G) + d] \cong  \bigoplus_{E' \in \irr(W^{{\H}})}	\langle \Ind^{W}_{W_{{\Ll}}} E ,	\Ind^{W}_{W^{{\H}}}E'  \rangle_{W} (\Aa^{\Ql}_{E'})_{\vert {\H}_{uni}}[-\dim(\T)].\]
We consider the restriction to $({s} u_\Cc)_\G$. By the same argument as in \cite[Proof of Thm.~2.4]{lusztigRestrictionCharacterSheaf2015}, we need to consider only the character sheaves of $\H$ which correspond under the Springer correspondence to the unipotent class $6631$, that is character sheaves such that $(\Aa^{\Ql}_{E'})_{\H_{uni}} = IC(\overline{(u)_\H}, \mathcal{E'})[\dim(T)-\dim((u)_\H)]$ for $E' \in \irr(W^{{\H}})$ and $\mathcal{E'}$ a local system on $(u)_\H$. Indeed, if $v \in \H$ is unipotent such that $(u)_\H \not \subseteq \overline{(v)_\H}$, then $IC(\overline{(v)_\H}, \mathcal{E'})_{\vert (u)_\H}= 0$ for $\mathcal{E'}$ a local system on $(v)_\H$. On the other hand, if $(u)_\H \subseteq \overline{(v)_\H}- (v)_\H$, then $(u)_\G \subseteq \overline{(v)_\G} - (v)_\G$. By definition of the unipotent support, we must have $s^*((\Aa_E)_{\vert s (v)_\H}) = 0$. Thus the character sheaf of the form $\Aa^{\Ql}_{E'} = IC(\overline{(v)_\H}, \mathcal{E'})[\dim(T)-\dim((u)_\H)]$ can not appear in the decomposition of $s^*((\Aa_E)_{\vert s \H_{uni}})$. 
\\ 

By the Springer correspondence, there is only one character $E' \in \irr(W^{{\H}})$ such that $\Aa^{\Ql}_{E'}[-\dim(\T)]$ is of the form $IC(\overline{(u)_\H}, \mathcal{E'})[\dim (u)_\H]$ for $E' \in \irr(W^{{\H}})$ and $\mathcal{E'}$ a local system on $(u)_\H$. In that case, $\Aa^{\Ql}_{E'} = IC(\overline{(u)_\H}, \Ll_{trivial})[\dim (u)_\H]$ where $\Ll_{trivial}$ is the local system on $(u)_\H$ corresponding to the trivial character of $A_\H(u) = C_\H(u)/C^\circ_\H(u)$. Using CHEVIE, we conclude that $\langle \Ind^{W}_{W_{{\Ll}}} (\phi_{30,15},111) ,	\Ind^{W}_{W^{{\H}}}E'  \rangle_{W} = 0$, whence \[\Aa_{(s u)_\H} = 0.\]

We see that there is an $F$-stable character sheaf $\mathcal{A}$ with unipotent support $\Cc$ such that 
\begin{itemize}
	\item $\mathcal{A}_{\vert ({s} u_\Cc)_{C_\G^\circ({s})}} = 0$, and 
	\item $\mathcal{A}_{\vert(u_\Cc)_\G}[-\dim(\Cc)-\dim(\T)]$ is a local system corresponding to the trivial character of $A_\G(u_\Cc)$. 
\end{itemize}
Therefore, we can apply the same proof as for \cite[Prop.~8.8]{brunatUnitriangularShapeDecomposition2020}, and we get that for all $[b,\phi] \in \Mm(A)$ \[\langle F^G_{[b,\phi]}, D_\G(\chi_\mathcal{A}) \rangle = \begin{cases}
	x_\mathcal{A}  &\text{ if } [b,\phi] =[1,1] \\
	0 &\text{ otherwise,}
\end{cases}\]
for some $x_\mathcal{A} \in \C^\times$.

\subsection{The unipotent conjugacy class $E_7(a_5)$ when $\ell = 2$} 
%
 We fix the setting in the case where the $F$-stable unipotent class is $\Cc = E_7(a_5)$. We choose $t \in \T^*$ such that $C_{\G^*}(t)$ is of type $E_6 \times A_2$ and $v \in C_{\G^*}(t)$ lies in the unipotent class $D_4(a_1),11$ of $E_7 \times A_1$.

\subsubsection{Admissible covering}
%\footnote{with the help of Jay Taylor}.\\
%We use the notation from \cite[$\S$ 10]{brunatUnitriangularShapeDecomposition2020}.\\
We fix $\mathbf{M}$ the Levi subgroup of $\G$ of type $E_7$. We fix an element $u_\Cc \in \mathbf{M}^F$ such that $(u_\Cc)_\G$ is the unipotent conjugacy class $E_7(a_5)$ and $F$ acts trivially on $A_\mathbf{M}(u_\Cc) \cong S_3$. We write $\Cc_{\mathbf{M}} \defeq (u_\Cc)_{\mathbf{M}}$. Then the unipotent conjugacy class $\Cc_{\mathbf{M}}$ is distinguished in $\mathbf{M}$. We fix a cocharacter $\lambda \in Y_{\mathcal{D}}^{\mathbf{M}}(u)^F$. By the same reasoning as in \cite[$\S$ 10.4]{brunatUnitriangularShapeDecomposition2020}, the group $A = C_{\L_{\mathbf{M}}(\lambda)}(u_\Cc)$ is an admissible covering of $A_{\mathbf{M}}(u_\Cc)$. Then, by the argument at the end of \cite[$\S$ 10.5]{brunatUnitriangularShapeDecomposition2020}, where they apply \cite[Lem.~4.4]{brunatUnitriangularShapeDecomposition2020}, the admissible pair $(A,\lambda)$ is also an admissible covering for $A_\G(u_\Cc)$. 
Observe that $$A \cong A_\G(u_\Cc) \cong \Omega_{C_{\G^*(t)},(v)_{C_{\G^*}(t)}}$$ and if $\ell = 2$, then $ A \cong \Omega^\ell_{\G,\Cc}.$
 

\begin{rmk} 
	%We first fix $a = \omega_{\alpha_1}(1/2) \in \T_0$ a semisimple and isolated involution of $G$ such that $C_\G^\circ(a)$ is of type $D_8$. 
	Observe that by \cite[Thm. 1]{mcninchComponentGroupsUnipotent2003} we have, $$A_\G(u_\Cc) \cong \langle \omega_{\alpha_1}(1/2)^{h_1}C_\G^\circ(u_\Cc), \omega_{\alpha_2}(1/3)^{h_2}C_\G^\circ(u_\Cc) \rangle$$ for some $h_1,h_2 \in \G$.  
\end{rmk}




\subsubsection{Character sheaves }
We fix $\Ll \defeq \alpha(s) \in \mathcal{S}(\T)$.
We consider a principal series character sheaf of $\G$ coming from $\mathcal{L}$ with unipotent support $E_7(a_5)$. Thanks to Lusztig's map (\cite[Thm.~10.7]{lusztigUnipotentSupportIrreducible1992}), we choose the one corresponding to the character of $W_\Ll$ denoted by $\phi_{315,16},11$. In order to apply the same argument as in the proof of \cite[Prop.~8.8]{brunatUnitriangularShapeDecomposition2020}, we need to compute the value of the characteristic function of $\Aa \defeq \Aa^\Ll_{\phi_{315,16},11}$ on the conjugacy classes $(au_\Cc)_{C^\circ_\G(a)}$ for each $a \in A$.\\ 

%Firstly, \[(A)_{(u)_\G}[-\dim(\Cc)-\dim(\T)] =  \Ll_{trivial}. \]

Let's look at the case where $a$ in an involution. Then, there exists $x \in \G$ such that $a^x = \omega_{\alpha_1}(1/2) \in \T$.  We fix ${s} \defeq \omega_{\alpha_1}(1/2) \in \T $ such that $\H \defeq C_\G({s})$ is of type $D_8$. Thanks to Algorithm 5.2 in \cite{brunatUnitriangularShapeDecomposition2020}, since only one unipotent class of $\H$ fuses into $\Cc$, we know that $u \defeq u_\Cc^x$ lies in the unipotent class $7522$ of $\H$ which fuses into $E_7(a_5)$. \\
We want to compute the restriction of the previous character sheaf to the mixed conjugacy class $(s u)_\H$.
We compute $W^{\H}\backslash W /W_{\Ll} = \{1,g\}$ for some $g \in W$. The group $W^{\H} \cap W_{\Ll}$ is a Weyl group. On the other hand, $W^g_\Ll \defeq W^{\H^g} \cap W_{\Ll} $ is not a Weyl group and we have $W^g_\Ll/(W^g_\Ll)^\circ \cong C_2 \cong Z(\H^g)$. Thus, by Lemma \ref{lem_valchiz}, $\chi^s$ is the sign character. \\
%We want to compute the restriction of the previous character sheaf to the mixed conjugacy class $(s u)_\H$. By the same argument as before, we can consider only the character sheaves of $\H$ of the form $A^{\Ql}_{E'} = IC(\overline{(u)_\H},\mathcal{E'})$ for $E' \in \irr(W^{{\H}})$ and $\mathcal{E'}$ a local system on $(u)_\H$. \\
%We observe using CHEVIE that there is only one character $E' \in \irr(W^{{\H}})$ such that $A^{\Ql}_{E'}$ is of the form $IC(\overline{(u)_\H}, \mathcal{E'})$ for $E' \in \irr(W^{{\H}})$ and $\mathcal{E'}$ a local system on $(u)_\H$. In that case, $A^{\Ql}_{E'} = IC(\overline{(u)_\H}, \Ll_{trivial})$ where $\Ll_{trivial}$ is the local system on $(u)_\H$ corresponding to the trivial character of $A_\H(u) = C_\H(u)/C^\circ_\H(u)$.\\
Using CHEVIE, we can compute that\footnote{if we did not tensor by the sign character when applying Proposition \ref{prop_formula}, we would have had $(\Aa)_{({s} u)_\H} \neq 0$} \[(\Aa)_{(s u)_{\H}} = 0. \] 

Lastly, we consider the case where $a$ has order $3$. By similar arguments as before, using CHEVIE, we compute that \[(\Aa_{(a u_\Cc)_{C_\G(a)}} = 0. \]
% There exists $x \in \G$ such that $a^x = \omega_{\alpha_2}(1/3) \in \T$. We fix ${s}' \defeq \omega_{\alpha_2}(1/3) \in \T$ semisimple such that $\H' \defeq C_\G(\defeq') $ is of type $A_8$. Thanks to Algorithm 5.2 in \cite{brunatUnitriangularShapeDecomposition2020}, since only one unipotent class of $\H$ fuses into $\Cc$, we know that $u \defeq u_\Cc^x$ lies in the unipotent class $63$ of $\H$ which fuses into $E_7(a_5)$. \\
%We set $W^{\H'}\backslash W /W_{\Ll} = \{1,g\}$ for some $g \in W$. The groups $W^{\H'} \cap W_{\Ll}$ and $W^{\H'^g} \cap W_{\Ll} $ are both Weyl groups. Therefore $\chi^{s}$ and $\chi^{s^g}$ are trivial, by Lemma \ref{lem_valchiz}. We can thus use the Mackey formula to simplify Proposition \ref{prop_formula}.\\
%We want to compute the restriction of the previous character sheaf to the mixed conjugacy class $({s}' u)_{\H'}$. We restrict our computation to the character sheaves of $\H'$ of the form $A^{\Ql}_{E'} = IC(\overline{(u)_{\H'}},\mathcal{E'})$ for $E' \in \irr(W^{{\H'}})$ and $\mathcal{E'}$ a local system on $(u)_{\H'}$. 


We see that there is an $F$-stable  character sheaf $\mathcal{A}$ with unipotent support $\Cc$ such that 
\begin{itemize}
	\item $\mathcal{A}_{\vert (a u_\Cc)_{C_\G^\circ({s})}} = 0$ if $a \neq 1$ for any $a \in A$.  
	\item $\mathcal{A}_{\vert(u_\Cc)_\G}[-\dim(\Cc)-\dim(\T)]$ is a local system corresponding to the trivial character of $A_\G(u_\Cc)$. 
\end{itemize}
Therefore, we can apply the same proof as for \cite[Prop.~8.8]{brunatUnitriangularShapeDecomposition2020}, and we get that for all $[b,\phi] \in \Mm(A)$ \[\langle F^G_{[b,\phi]}, D_\G(\chi_\mathcal{A}) \rangle = \begin{cases}
	x_\mathcal{A}  &\text{ if } [b,\phi] =[1,1] \\
	0 &\text{ otherwise,}
\end{cases}\]
for some $x_\mathcal{A} \in \C^\times$.\\


%For each simple root $\alpha \in \Delta$, we set $\omega_\alpha$ the fundamental dominant coweight corresponding to $\alpha$.
%We first fix $a = \omega_{\alpha_1}(1/2) \in \T_0$ a semisimple and isolated involution of $G$ such that $C_\G^\circ(a)$ is of type $D_8$. 

%Then for each $[a, \Phi_j] \in \Mm^\ell(A)$, we choose the unipotent character $\rho_{[a, \Psi_j]}$ such that $\rho^*_{[a, \Psi_j]} = \hat{K}_{(a,\psi_j)}$. Now let any $[b,\Phi_n],[a,\Psi_j] \in \Mm^\ell(A)$. If $b$ is not $A$-conjugate to $a$, then \[\langle \rho^*_{[b, \Phi_n]}, K_{[a,\Psi_i]} \rangle = 0.\] Else, there is $1 \leq i\leq s_a$ such that $[b,\Phi_n]= [a,\Psi_i]$ and we have \[\langle \rho^*_{[b, \Psi_n]}, K_{[a,\Psi_j]} \rangle = \begin{cases}
	%	0 \quad i<j,\\
	%	1 \quad i =j.\\
	%\end{cases}\]
	%
	%Thus, 
	
	
	
	%	For each $a \in A$, let $\{ \Psi_i \mid 1 \leq i \leq s_a\}$ be the set of all irreducible indecomposable characters of $C_A(a)$ and $\{ \psi_i \mid 1 \leq i \leq t_a \}$ be the set of all ordinary irreducible characters of $C_A(a)$. By the unitriangularity of the decomposition matrix of $C_A(a)$, we may assume that for $1 \leq i \leq j \leq s_a$,\[ d_{\psi_i,\Psi_j} =  \begin{cases}
		%	1 \text{ if } i = j, \\
		%	0 \text{ if } i <j.\end{cases}\]
	%	
	%	For $a \in A$, $\psi \in \irr(C_A(a))$ and $ \Psi$ the character of a projective indecomposable $kC_A(a)$-module, let us denote $\hat{K}^G_{(a,\Psi)}$ (resp. $\hat{K}^G_{(a,\psi)}$) for the projection of $K^G_{(a,\Psi)}$ (resp. $K^G_{(a,\psi)}$) on the space spanned by the unipotent characters such that their Alvis-Curtis dual has unipotent support $\mathcal{C}$ (alternatively with wave front set $\Cc$). 
	%	
	%	Firstly we observe that for any $1 \leq j \leq s_a$, we have  \[\hat{K}_{(a,\Psi_j)} = \sum_{1\leq t_a} d_{\psi_i,\Psi_j}\hat{K}_{(a,\psi_i)} = \hat{K}_{(a,\psi_j)} + \sum_{j< i \leq t_a} d_{\psi_i,\Psi_j}\hat{K}_{(a,\psi_i)}.\] 
	%	
	
	%Thus we can choose for each $[a, \Psi_j] \in \mathcal{M}^l(\Omega_{\G,u})$, we choose the projective $K_{(a,\Psi_j)}$ and the unipotent character $\hat{K}_{(a,\psi_j)}$.\\
	%We just need to check that $K_{(a,\Psi)}= K_{(b,\Phi)}$ if and only if $[a,\Psi] = [b,\Phi]$. However, if $K_{(a,\Psi)}= K_{(b,\Phi)}$, then $\hat{K}_{(a,\Psi)}= \hat{K}_{(b,\Psi)}$. Thus for each $\psi \in Irr(C_A(a))$, there must be $g \in A$ such that ${}^ga = b$, ${}^g\psi = \phi$ for a unique $\psi \in Irr(C_A(b))$ and $d_{\psi, \Psi} = d_{\phi, \Phi}$. Thus we may assume that for a fixed $g \in A$ ${}^ga =b$ and ${}^g\psi = \phi$. Then $\hat{K}_{(a,\Psi)}= \hat{K}_{({}^ga,{}^g\Psi)} = \hat{K}_{(b,{}^g\Psi)}$. So for all $\psi \in Irr(C_A(b))$ we must have $d_{\psi, {}^g\Psi}\hat{K}_{(b,\psi)} = d_{\psi, \Phi}\hat{K}_{(b,\psi)}$, whence $d_{\psi, {}^g\Psi}= d_{\psi, \Phi}$. Thus ${}^g\Psi = \Phi$ and $[a,\Psi] = [b,\Phi]$.\\
	
	
	
	%Let us now assume that $A$ is abelian. Firstly, we observe that for $[a, \phi] \in \mathcal{M}(A)$ such that $\hat{K}_{(a,\phi)} \neq 0$, then \[1 = \langle \hat{K}_{(a,\phi)}, \hat{K}_{(a,\phi)}\rangle = \frac{1}{|A|^2} \sum_{\substack{[b, \psi] \in \mathcal{M}(A)\\ z \in Z\\Z \subseteq Ker(\psi)}} \phi(z^{-1})\sgn(b)\sgn(bz)\zeta_{[b, \psi]}\zeta^{-1}_{[bz, \psi]}. \]
	%Firstly, we see that the sum does not depend on $a$, whence $\hat{K}_{(c,\phi)} \neq 0$ for any $c \in A$.
	%Then each term in the sum must be equal to $1$. In particular the values of $\phi$ are fixed on $Z$ ($\phi(z) = \sgn(1)\sgn(z)\zeta_{[1, 1]}\zeta^{-1}_{[z, 1]}$). 
	%Moreover, for $[a, \phi] \in \mathcal{M}(A)$ such that $\hat{K}_{(a,\phi)} \neq 0$ and for $[c, \chi] \in \mathcal{M}(A)$ such that $\hat{K}_{(c,\chi)} \neq 0$, 
	%\begin{align*}
	%		\langle \hat{K}_{(a,\phi)}, \hat{K}_{(c,\chi)}\rangle &= \frac{1}{|A|^2} \sum_{\substack{[b, \psi],[b', \psi'] \in \mathcal{M}(A)\\ Z \subseteq Ker(\psi) \cap2 Ker(\psi')\\ [\bar{b}, \bar{\psi}]=[\bar{b'}, \bar{\psi'}]}} \phi(b)\overline{\chi(b')\psi(a)}\psi'(c)\sgn(b)\sgn(b')\zeta_{[b, \psi]}\zeta^{-1}_{[b', \psi']},\\
	%		&= \frac{1}{|A|^2} \sum_{\substack{[b, \psi] \in \mathcal{M}(A)\\ z \in Z\\ Z \subseteq Ker(\psi)}} \phi(b)\overline{\chi(bz)\psi(a)}\psi(c)\sgn(b)\sgn(bz)\zeta_{[b, \psi]}\zeta^{-1}_{[bz, \psi]},\\
	%		&=\frac{1}{|A|^2} \sum_{\substack{[b, \psi] \in \mathcal{M}(A)\\ z \in Z\\ Z \subseteq Ker(\psi)}} \phi(b)\overline{\chi(bz)\psi(a)}\psi(c)\chi(z).
	%	\end{align*}
%Again this sum is either 0 or 1 and if it is $1$ then each term	of the sum must be $1$. In particular setting $\psi$ to be trivial, that $\phi =\chi$ and setting $b =1$, we observe that $a^{-1}c \in Ker(\psi)$ for all $\psi \in\irr(A)$ such that $Z \subseteq Ker(\psi)$. \\
%Observe that \begin{itemize}
	%	\item they are exactly $|\mathcal{M}(\Omega_u)|$ unipotent characters in this family, that is $|\Omega_u|^2 = \frac{|A|^2}{|Z|^2}$ as $\Omega_u$ is abelian. 
	%	\item They are at most $\frac{|A|}{|Z|}\frac{|A|}{\cap_{Z \subseteq Ker(\psi), \psi \in\irr(A) }Ker(\psi)}$ different $\hat{K}_{(a,\phi)}$ for $(a,\phi)$ in $\mathcal{M}(A)$.
	%\end{itemize}
	%However for each unipotent character $\rho$ we can find a unique $(a,\psi) \in\mathcal{M}(A)$ such that $\hat{K}_{(a,\psi)} = D_G(\rho).$
	%Thus by comparing size, we conclude that for $[a, \phi] \in \mathcal{M}(A)$ such that $\hat{K}_{(a,\phi)} \neq 0$ and for $[c, \chi] \in \mathcal{M}(A)$ such that $\hat{K}_{(c,\chi)} \neq 0$, $\hat{K}_{(a,\phi)}= \hat{K}_{(c,\chi)}$ if and only if $\phi =\chi$ and $a^{-1}c \in Z$, that is $\bar{a} = \bar{c}$.\\
	%
	%
	%Then for any unipotent character $\rho$, there is a unique $(b,\psi) \in \mathcal{M}(A)$ such that $\rho = \hat{K}_{(b,\psi)}$. Then for $(a, \Phi) \in \mathcal{M}^l(A)$, we have
	%\[\langle K_{(a,\Phi)}, \rho \rangle = \langle \hat{K}_{(a,\Phi)}, \hat{K}_{(b,\psi)} \rangle = \sum_{\phi \in Irr(A)} d_{\phi, \Phi}\langle \hat{K}_{(a,\phi)}, \hat{K}_{(b,\psi)} \rangle = \begin{cases}
		%d_{\psi, \Psi} \text{ if } \bar{a} = \bar{b} \\
		%0 \text{ else}.
		%\end{cases}\]
		%
		%In particular, $ \hat{K}_{(a,\Phi)} = 0$ if and only there is no $\psi \in \irr(A)$ such that $\psi(z) = \sgn(1)\sgn(z)\zeta_{[1, 1]}\zeta^{-1}_{[z, 1]}$ for all $z \in Z$ and $d_{\psi, \Psi} \neq 0.$ \\
		%For $(a, \Phi),(c,\chi) \in \mathcal{M}^l(A)$, we have $\hat{K}_{(a,\Phi)} = \hat{K}_{(c,\chi)} \neq 0$ if and only if $\bar{a} = \bar{c}$ and $\Phi =\chi.$ 
		%
		%\textcolor{red}{If $\psi(z) = \sgn(1)\sgn(z)\zeta_{[1, 1]}\zeta^{-1}_{[z, 1]}$ for all $z \in Z$ means that $Z \subseteq \psi$}. Then for each projective indecomposable of $\Omega_u \cong \frac{A}{Z}$, we can lift it to a projective indecomposable of $A$. Using the unitraingularity we will be done. 

==> centraltrans_principal.tex <==
\subsection{The principal series case}\label{subsec_principalserie}

In this subsection, we will only consider character sheaves which are constituent of the induction of a cuspidal character sheaf $K$ of a torus, and we assume that this torus is in fact $\T $. 
As in \cite[$\S$ 3.4]{taylorEvaluatingCharacteristicFunctions2014}, we can fix $$K = IC(\T ,{\Ll})[\dim\T ],$$ for ${\Ll} = \lambda^*(\mathcal{E}_{n,\psi}) \in \mathcal{S}(\T )$. \\

In this case, following \cite[Section 2]{lusztigCharacterValuesFinite1986}, we  precisely describe $\End(\Ind_\B^\G(K))$ and the isomorphism with the group algebra $W_{\Ll}$ over $\overline{\Q}_\ell$. We recall the induction diagram of the local system in that case:
\begin{center}
	\begin{tikzcd}
		\T & \G \times \T_{reg}\arrow[l, "\alpha"'] \arrow[r, "\beta"] & \G \times_\T \T_{reg} \arrow[r, "\delta"] & Y_{\T}
	\end{tikzcd}
\end{center}
with \begin{itemize}
	\item the set $\T_{reg} \defeq \{g \in \T \mid C^\circ_\G(g) = \T \}$ and the set $Y_{\T} \defeq \bigcup_{g \in \G}g\T_{reg}g^{-1}$,
	\item the set $\G \times_\T \T_{reg}$ is the quotient of $\G \times \T_{reg}$ by the $\T$-action $t.(g,m) = (gt^{-1}, tmt^{-1}) = (gt^{-1},m)$ for $t,m \in \T, g \in \G$,
	\item the map $\alpha$ is the projection on $\T$ of the second coordinate,
	\item the quotient map $\beta$,
	\item and the map $\delta: (g,m) \mapsto gmg^{-1}$ for $g \in \G, m \in \T_{reg}$.
\end{itemize}
Observe that $\overline{Y_\T} = \G$. \\

We define $\mathcal{A}_{\Ll} \defeq \End(\delta_*(\tilde{{\Ll}}))$.
For each $w \in W$, we also set $$\mathcal{A}_{{\Ll},w} \defeq \Hom(\ad(w^{-1})^*\tilde{{\Ll}},\tilde{{\Ll}}).$$ This vector space has dimension $1$ if and only if $\ad(w^{-1})^*{\Ll}\cong {\Ll}$ if and only if $w \in W_{\Ll}$. Otherwise it has dimension $0$. 
There is a natural pairing for $w,w' \in W_{\Ll}$:
\begin{align*}
	\mathcal{A}_{{\Ll},w} &\times \mathcal{A}_{{\Ll},w'} \to \mathcal{A}_{{\Ll},ww'} \\
	f \times g &\mapsto w'^*(f) \circ g.
\end{align*}
Since $\delta_*(\tilde{{\Ll}}) = \delta_*\left(\ad(w^{-1})^*\tilde{{\Ll}}\right)$, we obtain a natural isomorphism $$\mathcal{A}_{\Ll} \cong \bigoplus_{w \in W_{\Ll}}\mathcal{A}_{{\Ll},w}.$$

For $w \in W_{\Ll}$, we fix an isomorphism $\phi^{\Ll}_w: \ad(w^{-1})^*{\Ll}\to {\Ll}$ such that $(\phi^{\Ll}_w)_1$ is the identity. It induces an isomorphism $\tilde{\phi}^{\Ll}_w \in \mathcal{A}_{{\Ll},w}$. We then get an identification as follows 
$$\mathcal{A}_{{\Ll},w} = \Hom(\ad(w^{-1})^*\tilde{{\Ll}},\tilde{{\Ll}}) = \Ql\phi^{\Ll}_w \longleftrightarrow \Ql\phi^{\Ql}_w = \mathcal{A}_{\Ql,w}.$$

This gives an embedding of algebras $\mathcal{A}_{\Ll} \to \mathcal{A}_{\Ql}$.\\ Following \cite[$\S$ 2.4]{lusztigIntersectionCohomologyComplexes1984}, we fix a canonical basis $\{\theta_w \mid w \in W, \, \theta_w \in \mathcal{A}_{\Ql,w}\}$ such that $\theta_w\theta_{w'} = \theta_{ww'}$ for all $w,w' \in W$.  These elements $\theta_w$ might be regarded as basis elements for $\mathcal{A}_{\Ll}$. We write $\theta^{\Ll}_w$ for the element of $\mathcal{A}_{{\Ll},w}$ corresponding to $\theta_w$ under the identification above. Those isomorphisms $\theta^{\Ll}_w$ extend to an endomorphism of $IC(\overline{Y_{\T } },\delta_*(\tilde{{\Ll}}))$, that we denote by $\Theta^{\Ll}_w$.  
We then get a canonical isomorphism $\Ql\left[ W_{\Ll}\right] \cong \End(IC(\overline{Y_{\T }},\delta_*(\tilde{{\Ll}}))).$\\
In fact, by \cite[Thm. 6.2 and Cor. 6.9]{bonnafeActionsRelativeWeyl2003}, we may assume that $\theta_w = \tilde{\phi}^{\Ql}_w$ whence $\theta^{\Ll}_w = \tilde{\phi}^{\Ll}_w$.\\

Thanks to this construction, we can write \[\Ind_\P^\G(K) \cong \bigoplus_{E \in \irr(W_\Ll)} A^\Ll_E \otimes V_E,\] where $A^\Ll_E$ are the irreducible character sheaves in $\Ind_\P^\G(K)$ and $V_E = \Hom(A^\Ll_E,\Ind_\P^\G(K))$ are the irreducible $\Ql[W_\Ll]$-module.\\


We would like to consider translation of character sheaves by an element of the center of $\G$. For $z \in Z(\G) \cap \T$, we define $z: \T \to \T,\, t \mapsto zt$ for $t \in \T$.\\ 
Observe that $$z^*\Ll = \lambda^*t_{\lambda(z)}^*\mathcal{E}_{n,\psi} \cong \Ll.$$  Therefore we have $z^*K \cong IC(\T,z^*\Ll) \cong K$ and $z^*\Ind_\P^\G(K) \cong \Ind_\P^\G(IC(\T,z^*\Ll)) \cong \Ind_\P^\G(K)$. However, we might not have an isomorphism between $\left(A_E^\Ll\right)$ and $A_E^{z^*\Ll}$ for $E \in \irr(W_\Ll)$. 

\begin{lem}
	Let $z \in Z(\G)$, $w \in W_{\Ll}$, then
	$$\psi(\lambda_w(z))z^*(\phi^{{\Ll}}_w) = \phi^{z^*{\Ll}}_w \quad \text{ and } \,  \psi(\lambda_w(z))z^*(\tilde{\phi}^{{\Ll}}_w) = \tilde{\phi}^{z^*{\Ll}}_w.$$ 
\end{lem}
\begin{proof}
	Since $z \in Z(\G)$, we have $W_{z^*{\Ll}} = W_{{\Ll}}$ and $\phi^{z^*{\Ll}}_w$ is well-defined. 
	Since $z^*(\phi^{{\Ll}}_w) \in \mathcal{A}_{z^*{\Ll},w}$, the two isomorphisms $z^*(\phi^{{\Ll}}_w)$ and $\phi^{z^*{\Ll}}_w$ differ by a scalar. We can then just consider the stalks at $1$. 
	In other words, we need to compute $(\phi^{{\Ll}}_w)_z$. Passing from ${\Ll}_1$ to ${\Ll}_z = \left(z^*\Ll\right)_1$ is given by the isomorphism in Lemma \ref{lem_isostalks}. Indeed, we consider the isomorphism $\mu$ which is just multiplication by $\psi(\lambda(z)_n)$  We have the following diagram:
	\begin{center}
		\begin{tikzcd}
			(ad(w^{-1})^*{\Ll})_1 \arrow[rr, "(\phi_w^{\Ll})_1 = id"] \arrow[d, "\cdot \psi(\lambda_w(z)\lambda(z)_n)"'] &  & {\Ll}_1 \arrow[d, "\cdot \psi(\lambda(z)_n)"]    \\
			(ad(w^{-1})^*{\Ll})_z  \arrow[rr, "(\psi^{\Ll}_w)_z"']                                                 &  & {\Ll}_z 
		\end{tikzcd} 
	\end{center}
	Therefore $(\phi^{{\Ll}}_w)_z$ is simply multiplication by $ \phi(\lambda_w(z))^{-1}$ whence $\psi(\lambda_w(z))z^*(\phi^{{\Ll}}_w) = \phi^{z^*{\Ll}}_w$ and $\psi(\lambda_w(z))z^*(\tilde{\phi}^{{\Ll}}_w) = \tilde{\phi}^{z^*{\Ll}}_w$.   
\end{proof}

\begin{lem}\label{lem_translationCS}
	Let $z \in Z(\G)$, $E \in \irr(W_{\Ll})$ we have 
	\[A^{{\Ll}}_E = A^{z^*{\Ll}}_{E\cdot \chi^z},\]
	and $\chi^z: W'_{\Ll} \to \overline{\Q}_\ell$ is given by $w \mapsto \psi(\lambda_w(z))$. 
\end{lem}

\begin{proof}	
	For $w \in W_{\Ll}$, we can define two embeddings of  $\mathcal{A}_{z^*{\Ll},w}$ into $\mathcal{A}_{\Ql,w}$: the first one being the usual one identifying $\phi^{z^*{\Ll}}_w$ with $\phi^{\Ql}_w$ and the second one identifying $z^*(\phi^{{\Ll}}_w)$ with $\phi^{\Ql}_w$. So we get two isomorphisms between $\Ql\left[ W_{\Ll}\right] $ and $ \End(IC(\overline{Y_{\T}},\delta_*(\tilde{z^*{\Ll}}))).$ From the previous lemma, we see that they differ by multiplication $\psi(\lambda_w(z))$. We define $\chi^z: W_\Ll \to \Ql$ by $w \mapsto \psi(\lambda_w(z))$ for any $w \in W_\Ll$.  One hand we have, 
	%Let's fix $E_0 \in \irr(\End(IC(\overline{Y_{\T}},\delta_*(\tilde{{\Ll}}))))$ such that it corresponds under the second isomorphism to $E_1 \in \irr(W_{\Ll})$ .
	\begin{align*}
		A^{{\Ll}}_E &\cong \Hom_{\End(IC(\overline{Y_{\T  }},\delta_*(\tilde{{\Ll}})))}\left(E, IC\left(\overline{Y_{\T  }},\delta_*(\tilde{{\Ll}})\right)\right)&\\
		&\cong \Hom_{W_{\Ll}}\left(E, IC\left(\overline{Y_{\T  }},\delta_*(\tilde{{\Ll}})\right)\right) \quad &(\phi^{{\Ll}}_w \leftrightarrow \phi^{\Ql}_w)\\
		& \cong z^*\Hom_{W_{\Ll}}(E,z^*IC(\overline{Y_{\T  }},\delta_*(\tilde{{\Ll}}))) \quad &(z^*\phi^{{\Ll}}_w \leftrightarrow \phi^{\Ql}_w) \\
		& \cong \Hom_{W_{\Ll}}(E,IC(\overline{Y_{\T  }},\delta_*(\tilde{z^*{\Ll}}))) &\\
	\end{align*}
	
	On the other hand, for $E' \in \irr(W_\Ll)$, we have 
	\begin{align*}
		A^{z^*{\Ll}}_{E'} &\cong z^*\Hom_{\End(IC(\overline{Y_{\T  }},\delta_*(\tilde{z^*{\Ll}})))}\left(E', IC\left(\overline{Y_{\T  }},\delta_*(\tilde{z^*{\Ll}})\right)\right)&\\
		&\cong \Hom_{W_{\Ll}}(E',IC(\overline{Y_{\T }},\delta_*(\tilde{z^*{\Ll}})))  &(\phi^{z^*{\Ll}}_w = \chi^z(w)z^*\phi^{{\Ll}}_w \leftrightarrow \phi^{\Ql}_w)	\\
		&\cong \Hom_{W_{\Ll}}(E'\cdot (\chi^z)^{-1},IC(\overline{Y_{\T }},\delta_*(\tilde{z^*{\Ll}}))).  &(z^*\phi^{{\Ll}}_w \leftrightarrow \phi^{\Ql}_w)	
	\end{align*}
	We conclude that $A^{{\Ll}}_E = A^{z^*{\Ll}}_{E'}$ if and only if $E' = E \cdot \chi^z$
\end{proof}

==> centraltrans_principal__1_.tex <==
\subsection{The principal series case}\label{subsec_principalserie}

In this subsection, we will only consider character sheaves which are constituent of the induction of a cuspidal character sheaf $K$ of a torus, and we assume that this torus is in fact $\T $. 
As in \cite[$\S$ 3.4]{taylorEvaluatingCharacteristicFunctions2014}, we can fix $$K = IC(\T ,{\Ll})[\dim\T ],$$ for ${\Ll} = \lambda^*(\mathcal{E}_{n,\psi}) \in \mathcal{S}(\T )$. \\

In this case, following \cite[Section 2]{lusztigCharacterValuesFinite1986}, we  precisely describe $\End(\Ind_\B^\G(K))$ and the isomorphism with the group algebra $W_{\Ll}$ over $\overline{\Q}_\ell$. We recall the induction diagram of the local system in that case:
\begin{center}
	\begin{tikzcd}
		\T & \G \times \T_{reg}\arrow[l, "\alpha"'] \arrow[r, "\beta"] & \G \times_\T \T_{reg} \arrow[r, "\delta"] & Y_{\T}
	\end{tikzcd}
\end{center}
with \begin{itemize}
	\item the set $\T_{reg} \defeq \{g \in \T \mid C^\circ_\G(g) = \T \}$ and the set $Y_{\T} \defeq \bigcup_{g \in \G}g\T_{reg}g^{-1}$,
	\item the set $\G \times_\T \T_{reg}$ is the quotient of $\G \times \T_{reg}$ by the $\T$-action $t.(g,m) = (gt^{-1}, tmt^{-1}) = (gt^{-1},m)$ for $t,m \in \T, g \in \G$,
	\item the map $\alpha$ is the projection on $\T$ of the second coordinate,
	\item the quotient map $\beta$,
	\item and the map $\delta: (g,m) \mapsto gmg^{-1}$ for $g \in \G, m \in \T_{reg}$.
\end{itemize}
Observe that $\overline{Y_\T} = \G$. \\

We define $\mathcal{A}_{\Ll} \defeq \End(\delta_*(\tilde{{\Ll}}))$.
For each $w \in W$, we also set $$\mathcal{A}_{{\Ll},w} \defeq \Hom(\ad(w^{-1})^*\tilde{{\Ll}},\tilde{{\Ll}}).$$ This vector space has dimension $1$ if and only if $\ad(w^{-1})^*{\Ll}\cong {\Ll}$ if and only if $w \in W_{\Ll}$. Otherwise it has dimension $0$. 
There is a natural pairing for $w,w' \in W_{\Ll}$:
\begin{align*}
	\mathcal{A}_{{\Ll},w} &\times \mathcal{A}_{{\Ll},w'} \to \mathcal{A}_{{\Ll},ww'} \\
	f \times g &\mapsto w'^*(f) \circ g.
\end{align*}
Since $\delta_*(\tilde{{\Ll}}) = \delta_*\left(\ad(w^{-1})^*\tilde{{\Ll}}\right)$, we obtain a natural isomorphism $$\mathcal{A}_{\Ll} \cong \bigoplus_{w \in W_{\Ll}}\mathcal{A}_{{\Ll},w}.$$

For $w \in W_{\Ll}$, we fix an isomorphism $\phi^{\Ll}_w: \ad(w^{-1})^*{\Ll}\to {\Ll}$ such that $(\phi^{\Ll}_w)_1$ is the identity. It induces an isomorphism $\tilde{\phi}^{\Ll}_w \in \mathcal{A}_{{\Ll},w}$. We then get an identification as follows 
$$\mathcal{A}_{{\Ll},w} = \Hom(\ad(w^{-1})^*\tilde{{\Ll}},\tilde{{\Ll}}) = \Ql\phi^{\Ll}_w \longleftrightarrow \Ql\phi^{\Ql}_w = \mathcal{A}_{\Ql,w}.$$

This gives an embedding of algebras $\mathcal{A}_{\Ll} \to \mathcal{A}_{\Ql}$.\\ Following \cite[$\S$ 2.4]{lusztigIntersectionCohomologyComplexes1984}, we fix a canonical basis $\{\theta_w \mid w \in W, \, \theta_w \in \mathcal{A}_{\Ql,w}\}$ such that $\theta_w\theta_{w'} = \theta_{ww'}$ for all $w,w' \in W$.  These elements $\theta_w$ might be regarded as basis elements for $\mathcal{A}_{\Ll}$. We write $\theta^{\Ll}_w$ for the element of $\mathcal{A}_{{\Ll},w}$ corresponding to $\theta_w$ under the identification above. Those isomorphisms $\theta^{\Ll}_w$ extend to an endomorphism of $IC(\overline{Y_{\T } },\delta_*(\tilde{{\Ll}}))$, that we denote by $\Theta^{\Ll}_w$.  
We then get a canonical isomorphism $\Ql\left[ W_{\Ll}\right] \cong \End(IC(\overline{Y_{\T }},\delta_*(\tilde{{\Ll}}))).$\\
In fact, by \cite[Thm. 6.2 and Cor. 6.9]{bonnafeActionsRelativeWeyl2003}, we may assume that $\theta_w = \tilde{\phi}^{\Ql}_w$ whence $\theta^{\Ll}_w = \tilde{\phi}^{\Ll}_w$.\\

Thanks to this construction, we can write \[\Ind_\P^\G(K) \cong \bigoplus_{E \in \irr(W_\Ll)} A^\Ll_E \otimes V_E,\] where $A^\Ll_E$ are the irreducible character sheaves in $\Ind_\P^\G(K)$ and $V_E = \Hom(A^\Ll_E,\Ind_\P^\G(K))$ are the irreducible $\Ql[W_\Ll]$-module.\\


We would like to consider translation of character sheaves by an element of the center of $\G$. For $z \in Z(\G) \cap \T$, we define $z: \T \to \T,\, t \mapsto zt$ for $t \in \T$.\\ 
Observe that $$z^*\Ll = \lambda^*t_{\lambda(z)}^*\mathcal{E}_{n,\psi} \cong \Ll.$$  Therefore we have $z^*K \cong IC(\T,z^*\Ll) \cong K$ and $z^*\Ind_\P^\G(K) \cong \Ind_\P^\G(IC(\T,z^*\Ll)) \cong \Ind_\P^\G(K)$. However, we might not have an isomorphism between $\left(A_E^\Ll\right)$ and $A_E^{z^*\Ll}$ for $E \in \irr(W_\Ll)$. 

\begin{lem}
	Let $z \in Z(\G)$, $w \in W_{\Ll}$, then
	$$\psi(\lambda_w(z))z^*(\phi^{{\Ll}}_w) = \phi^{z^*{\Ll}}_w \quad \text{ and } \,  \psi(\lambda_w(z))z^*(\tilde{\phi}^{{\Ll}}_w) = \tilde{\phi}^{z^*{\Ll}}_w.$$ 
\end{lem}
\begin{proof}
	Since $z \in Z(\G)$, we have $W_{z^*{\Ll}} = W_{{\Ll}}$ and $\phi^{z^*{\Ll}}_w$ is well-defined. 
	Since $z^*(\phi^{{\Ll}}_w) \in \mathcal{A}_{z^*{\Ll},w}$, the two isomorphisms $z^*(\phi^{{\Ll}}_w)$ and $\phi^{z^*{\Ll}}_w$ differ by a scalar. We can then just consider the stalks at $1$. 
	In other words, we need to compute $(\phi^{{\Ll}}_w)_z$. Passing from ${\Ll}_1$ to ${\Ll}_z = \left(z^*\Ll\right)_1$ is given by the isomorphism in Lemma \ref{lem_isostalks}. Indeed, we consider the isomorphism $\mu$ which is just multiplication by $\psi(\lambda(z)_n)$  We have the following diagram:
	\begin{center}
		\begin{tikzcd}
			(ad(w^{-1})^*{\Ll})_1 \arrow[rr, "(\phi_w^{\Ll})_1 = id"] \arrow[d, "\cdot \psi(\lambda_w(z)\lambda(z)_n)"'] &  & {\Ll}_1 \arrow[d, "\cdot \psi(\lambda(z)_n)"]    \\
			(ad(w^{-1})^*{\Ll})_z  \arrow[rr, "(\psi^{\Ll}_w)_z"']                                                 &  & {\Ll}_z 
		\end{tikzcd} 
	\end{center}
	Therefore $(\phi^{{\Ll}}_w)_z$ is simply multiplication by $ \phi(\lambda_w(z))^{-1}$ whence $\psi(\lambda_w(z))z^*(\phi^{{\Ll}}_w) = \phi^{z^*{\Ll}}_w$ and $\psi(\lambda_w(z))z^*(\tilde{\phi}^{{\Ll}}_w) = \tilde{\phi}^{z^*{\Ll}}_w$.   
\end{proof}

\begin{lem}\label{lem_translationCS}
	Let $z \in Z(\G)$, $E \in \irr(W_{\Ll})$ we have 
	\[A^{{\Ll}}_E = A^{z^*{\Ll}}_{E\cdot \chi^z},\]
	and $\chi^z: W'_{\Ll} \to \overline{\Q}_\ell$ is given by $w \mapsto \psi(\lambda_w(z))$. 
\end{lem}

\begin{proof}	
	For $w \in W_{\Ll}$, we can define two embeddings of  $\mathcal{A}_{z^*{\Ll},w}$ into $\mathcal{A}_{\Ql,w}$: the first one being the usual one identifying $\phi^{z^*{\Ll}}_w$ with $\phi^{\Ql}_w$ and the second one identifying $z^*(\phi^{{\Ll}}_w)$ with $\phi^{\Ql}_w$. So we get two isomorphisms between $\Ql\left[ W_{\Ll}\right] $ and $ \End(IC(\overline{Y_{\T}},\delta_*(\tilde{z^*{\Ll}}))).$ From the previous lemma, we see that they differ by multiplication $\psi(\lambda_w(z))$. We define $\chi^z: W_\Ll \to \Ql$ by $w \mapsto \psi(\lambda_w(z))$ for any $w \in W_\Ll$.  One hand we have, 
	%Let's fix $E_0 \in \irr(\End(IC(\overline{Y_{\T}},\delta_*(\tilde{{\Ll}}))))$ such that it corresponds under the second isomorphism to $E_1 \in \irr(W_{\Ll})$ .
	\begin{align*}
		A^{{\Ll}}_E &\cong \Hom_{\End(IC(\overline{Y_{\T  }},\delta_*(\tilde{{\Ll}})))}\left(E, IC\left(\overline{Y_{\T  }},\delta_*(\tilde{{\Ll}})\right)\right)&\\
		&\cong \Hom_{W_{\Ll}}\left(E, IC\left(\overline{Y_{\T  }},\delta_*(\tilde{{\Ll}})\right)\right) \quad &(\phi^{{\Ll}}_w \leftrightarrow \phi^{\Ql}_w)\\
		& \cong z^*\Hom_{W_{\Ll}}(E,z^*IC(\overline{Y_{\T  }},\delta_*(\tilde{{\Ll}}))) \quad &(z^*\phi^{{\Ll}}_w \leftrightarrow \phi^{\Ql}_w) \\
		& \cong \Hom_{W_{\Ll}}(E,IC(\overline{Y_{\T  }},\delta_*(\tilde{z^*{\Ll}}))) &\\
	\end{align*}
	
	On the other hand, for $E' \in \irr(W_\Ll)$, we have 
	\begin{align*}
		A^{z^*{\Ll}}_{E'} &\cong z^*\Hom_{\End(IC(\overline{Y_{\T  }},\delta_*(\tilde{z^*{\Ll}})))}\left(E', IC\left(\overline{Y_{\T  }},\delta_*(\tilde{z^*{\Ll}})\right)\right)&\\
		&\cong \Hom_{W_{\Ll}}(E',IC(\overline{Y_{\T }},\delta_*(\tilde{z^*{\Ll}})))  &(\phi^{z^*{\Ll}}_w = \chi^z(w)z^*\phi^{{\Ll}}_w \leftrightarrow \phi^{\Ql}_w)	\\
		&\cong \Hom_{W_{\Ll}}(E'\cdot (\chi^z)^{-1},IC(\overline{Y_{\T }},\delta_*(\tilde{z^*{\Ll}}))).  &(z^*\phi^{{\Ll}}_w \leftrightarrow \phi^{\Ql}_w)	
	\end{align*}
	We conclude that $A^{{\Ll}}_E = A^{z^*{\Ll}}_{E'}$ if and only if $E' = E \cdot \chi^z$
\end{proof}

==> centraltrans_unip__1_.tex <==



%In this subsection, we will only consider character sheaves coming from the principal series. We can fix $\Ll =  \lambda^*(\mathcal{E}_{n,\psi}) \in \mathcal{S}(\T)$. We consider the cupisdal character sheaf
%$$K = IC(T , \Ll)[\dim \T ]$$ 
%and the irreducible constituents of its induction. 
%
%In this case, f
%Following \cite[Section 2]{lusztigCharacterValuesFinite1986}, we  precisely describe $\End(\Ind_\B^\G(K))$ and the isomorphism with the group algebra $\Ql[W_{\Ll}]$.  We recall the induction diagram of the local system in that case:
%\begin{center}
%	\begin{tikzcd}
%		\T & \G \times \T_{reg}\arrow[l, "\alpha"'] \arrow[r, "\beta"] & \G \times_\T \T_{reg} \arrow[r, "\delta"] & Y_{\T}
%	\end{tikzcd}
%\end{center}
%with \begin{itemize}
%	\item the set $\T \defeq \{g \in \T \mid C^\circ_\G(g) = \T \}$ and the set $Y_{\T} \defeq \bigcup_{g \in \G}g\T_{reg}g^{-1}$,
%	\item the set $\G \times_\L\T \T_{reg}$, quotient of $\G \times \T_{reg}$ by the $\T$-action $t.(g,a) = (gt^{-1}, tat^{-1})$ for $t \in \T, g \in \G$ and $a \in \T_{reg}$,
%	\item the map $\alpha$ which is the projection on $\T$ of the second coordinate,
%	\item the quotient map $\beta$,
%	\item and the map $\delta: (g,a) \mapsto gag^{-1}$ for $g \in \G, a \in \T_{reg}$.
%\end{itemize}
%%
%Let $\Ee \boxtimes 1$ be the local system on $CZ^\circ(\L)$ which is the inverse image of $\Ee$ under the map $CZ^\circ(\L) \to C, uz \mapsto u$ for $u \in C$ and $z \in Z^\circ(\L)$. Then there is a canonical local system $\tilde{\Ee}$ on $\G \times_\L CZ^\circ(\L)_{reg}$ such that $\beta^*(\tilde{\Ee}) = \alpha^*(\Ee \boxtimes 1).$ \\
%Let $\tilde{\Ll}$ be the local system on $\G \times_\L CZ^\circ(\L)_{reg}$ which is the inverse image of $\Ll$ under the map $\G \times_\L CZ^\circ(\L)_{reg} \to Z^\circ(\L), (g,a) \mapsto a_s$ for $g \in \G$ and $a \in CZ^\circ(\L)_{reg}.$
%Then $\tilde{\Ee} \otimes \tilde{\Ll}$ is a local system on $\G \times_\L CZ^\circ(\L)_{reg}$. Moreover, there is a canonical isomorphism  \[IC(\overline{Y_{\L,\Sigma}},\delta_*(\tilde{\Ee \otimes \Ll}))[\dim Y_{\L,\Sigma}] \cong IC(\overline{Y_{\L,\Sigma}},\delta_*(\tilde{\Ee}) \otimes \delta_*(\tilde{\Ll}))[\dim Y_{\L,\Sigma}].\]



%
\subsection{Central translation of character sheaves with unipotent support}\label{sect_centraltrans}
We would like to consider translation of character sheaves by an element of the center of $\G$. For $z \in  Z(\G)$, we define the translation $z: \T \to \T,\, t \mapsto zt$ for $t \in \T$.

\subsubsection{Translation of Kummer systems}
We want to get a better understanding of the isomorphism $\phi^\Ll_w : \ad(w^{-1})^*\Ll \to \Ll$ for $\Ll \in \mathcal{S}(\T)$ and $w \in W_\Ll$. 


We fix $n \in \N$ and $c \in k^\times$. The stalk $\left(\left(\rho_n\right)_*\Ql\right)_c$ can be seen as the $n$-dimensional $\Ql$-vector space $\Ql[\rho_n^{-1}(c)]$, with action of $\mu_n$  on $\rho_n^{-1}(c)$ by multiplication. In that setting, $\left(\mathcal{E}_{n,\psi}\right)_c$ is the $\Ql$-vector subspace of dimension one on which the action of $x \in \mu_n$ is simply multiplication by $\psi(x)$. \\
We start by a few observations, defining some morphisms and keeping track of their restriction to the stalks. Fix $\lambda,\gamma \in X(\T)$. Firstly, we have a $\mu_n$-equivariant morphism: \[(\lambda\gamma)^*\left(\rho_n\right)_*\Ql \to (\lambda)^*\left(\rho_n\right)_*\Ql \otimes_{\mu_n}(\gamma)^*\left(\rho_n\right)_*\Ql,\]
On the stalk $t \in \T$, we get a morphism of $\mu_n$-modules from $\Ql[\rho_n^{-1}(\lambda(t)\gamma(t))]$  to $\Ql[\rho_n^{-1}(\lambda(t))] \otimes_{\mu_n} \Ql[\rho_n^{-1}(\gamma(t))].$\\ 
Now, we denote by $\underline{\Ql[\mu_n]}_V$ the constant sheaf on a variety $V$. The adjunction $\left(\rho_n\right)^*\left(\rho_n\right)_*\Ql\to \Ql$ is given by the $\mu_n$-equivariant isomorphism: \[\left(\rho_n\right)^*\left(\rho_n\right)_*\Ql \to \underline{\Ql[\mu_n]}_{k^\times}.\] Taking the pullback by $\gamma$, we get a $\mu_n$-equivariant morphism \[(\gamma^n)^*\left(\rho_n\right)_*\Ql = \gamma^*\left(\rho_n\right)^*\left(\rho_n\right)_*\Ql \to \gamma^*\underline{\Ql[\mu_n]}_{k^\times} \to \underline{\Ql[\mu_n]}_{\T}. \] 
On the stalk at $t \in \T$, we get an isomorphism of $\mu_n$-modules from $\Ql[\rho_n^{-1}(\gamma^n(t))] = \Ql[\gamma(t)\mu_n]$  to $\Ql[\mu_n],$ by multiplication by $\gamma^{-1}(t)$. \\
Combining the two previous $\mu_n$-equivariant morphisms, we get 
\[(\lambda\gamma^n)^*\left(\rho_n\right)_*\Ql \to (\lambda)^*\left(\rho_n\right)_*\Ql \otimes_{\mu_n}(\gamma^n)^*\left(\rho_n\right)_*\Ql \to (\lambda)^*\left(\rho_n\right)_*\Ql \otimes_{\mu_n}\underline{\Ql[\mu_n]}_{\T} \to (\lambda)^*\left(\rho_n\right)_*\Ql.\]
On the stalk $t \in \T$, we get a morphism of $\mu_n$-modules from $\Ql[\rho_n^{-1}(\lambda(t)\gamma^n(t))] = \Ql[\gamma(t)\rho_n^{-1}(\lambda(t))]$ to $\Ql[\rho_n^{-1}(\lambda(t))],$ given by multiplication by $\gamma^{-1}(t)$. \\
This  $\mu_n$-equivariant morphism restricts to an isomorphism:
\[\nu_{\lambda,\gamma,n}: (\lambda\gamma^n)^*\Ee_{n,\psi} \to \lambda^*\Ee_{n,\psi}.\]  Let  $t \in \T$ such that $t^n =1$. The definition of $\Ee_{n,\psi}$ implies that the isomorphism $\left(\nu_{\lambda,\gamma,n}\right)_t$ of $\mu_n$-modules from $\left(\Ee_{n,\psi}\right)_{\lambda(t)} \subseteq \Ql[\rho_n^{-1}(\lambda(t))]$ to $\left(\Ee_{n,\psi}\right)_{\lambda(t)} \subseteq \Ql[\rho_n^{-1}(\lambda(t))]$ is in fact given by multiplication by $\psi(\gamma(t)^{-1})$. More generally, since we always have $\lambda^*\Ee_{n,\psi}$ isomorphic to $(\lambda^m)^*\Ee_{nm,\psi}$ for all $m \in\N$, for any element $t \in \T$ of finite order, the isomorphism $\left(\nu_{\lambda,\gamma,n}\right)_t$ of $\mu_n$-modules is simply  multiplication by $\psi(\gamma(t)^{-1}).$\\

We can now consider the particular case of the isomorphism between $ \ad(w^{-1})^*\Ll \to \Ll$ for $\Ll \in \mathcal{S}(\T)$ and $w \in W_\Ll$. The above discussion leads to the following result:
\begin{lem}\label{lem_defisoadw}
	Let $\Ll = \lambda^*\Ee_{n,\psi} \in \mathcal{S}(\T)$ for $n \in \N$ and $\lambda \in X(\T)$. Let $w \in W_\Ll$. Recall that there is $\lambda_w \in X(\T)$ such that $\lambda^w= \lambda\lambda_w^n$. Then $\phi_w^\Ll$ in in fact $\nu_{\lambda,\lambda_w,n}$. 
\end{lem}
\begin{proof}Since $\Ll$ is irreducible, it suffices to check that $ \left(\nu_{\lambda,\lambda_w,n}\right)_1$ is equal to $\left(\phi_w^\Ll\right)_1$, which is the identity. It clearly follows from the previous discussion.  
\end{proof}

\begin{lem}\label{lem_transphiLl}
	Let $z \in Z(\G)$, $w \in W_{\Ll}$, then there is $\lambda_w \in \Hom(\T, k^\times)$ depending on $\Ll$ such that
	$$\psi(\lambda_w(z))z^*(\phi^{{\Ll}}_w) = \phi^{z^*{\Ll}}_w \quad \text{ and } \,  \psi(\lambda_w(z))z^*(\tilde{\phi}^{{\Ll}}_w) = \tilde{\phi}^{z^*{\Ll}}_w.$$ 
\end{lem}
\begin{proof}
	We have $W_{z^*{\Ll}} = W_{{\Ll}}$ and $\phi^{z^*{\Ll}}_w$ is well-defined. 
	Since $z^*(\phi^{{\Ll}}_w) \in \mathcal{H}_{z^*{\Ll},w}$, the two isomorphisms $z^*(\phi^{{\Ll}}_w)$ and $\phi^{z^*{\Ll}}_w$ differ by a scalar. To determine it, it suffices to consider the stalks at $1$. On one hand, by definition, $\left(\phi^{z^*{\Ll}}_w\right)_1$ is the identity. On the other hand, by Lemma \ref{lem_defisoadw}, $\left(z^*(\phi^{{\Ll}}_w)\right)_1 = \left(\nu_{\lambda,\lambda_w,n}\right)_1$ is given by multiplication by $\psi(\lambda_w(z))^{-1}$ and we can conclude. 
\end{proof}



%Firstly, we consider the translation at the level of Kummer systems.  For $z \in k^\times$, we define the translation $z: k \to k,\, c \mapsto zc$ for $c \in k.$
%We consider isomorphisms between $\mathcal{E}_{n,\psi}$ and $z^*\left(\mathcal{E}_{n,\psi}\right)$.\\
%
%
%We fix $n,m \in \N$ and $c,z \in k^\times$ and define \[\mu_n^c \defeq \{x \in {k}^\times \mid x^n = c\}.\]  The stalk $\left(\left(\rho_n\right)_*\Ql\right)_c$ can be seen as an $n$-dimensional $\Ql$-vector space, with coordinates indexed by $\mu_n^c$. In that setting, $\left(\mathcal{E}_{n,\psi}\right)_c$ is a $\Ql$-vector space of dimension one on which the action of $x \in \mu_n$ is simply multiplication by $\psi(x)$.\\
%
% We consider some natural morphisms as well as their action on the stalks. Observe that all of the following morphisms commute with the action of $\mu_n$.
% \[\nu_{z,n}: (z^n)^*\left(\rho_n\right)_*\Ql \to \left(\rho_n\right)_*z^*\Ql \to \left(\rho_n\right)_*\Ql,\]
%where the first arrow is given by the change of basis and the second one by the fact that $z^*\Ql$ is in fact the constant sheaf. On the stalks, $(\nu_{z,n})_c: \left(\left(\rho_n\right)_*\Ql\right)_{z^nc} \to \left(\left(\rho_n\right)_*\Ql\right)_c$ sends the coordinate $zx$ to $x$ for $x \in \mu_n^c$. In particular, the action of $\mu_n$ on $\left(\rho_n\right)_*\Ql$ is given by the maps $\nu_{z,n}$ for $z \in \mu_n$. \\
%We also consider
%\[\iota: \left(\rho_{n}\right)_*\Ql \to \left(\rho_{nm}\right)_*\left(\rho_{m}\right)^* \Ql \to \left(\rho_{nm}\right)_*\Ql, \]
%where the first arrow is given by adjunction and the second by the fact that $\left(\rho_{m}\right)^* \Ql$ is the constant sheaf. On the stalks, it is simply the diagonal inclusion morphism given by pre-composition by $x \mapsto x^m$.
%Lastly, we set \[\eta: (\rho_m)^*(\rho_{mn})_*\Ql\to \left(\rho_{n}\right)_*\Ql, \]
%given by adjunction. On the stalks, it is given by the projection induced by $\mu_n^c \subseteq \mu_{nm}^{c^m}$. 
%
%Observe that $\eta_1 \circ \iota_1 = id$ but that it is not the case at the level of the sheaves. \\
%
%We now consider the case of Kummer local systems. We fix a field isomorphism $\Psi: \Ql \to \C$ and a group isomorphism $\beta: \T \to (k^\times)^r$ where $r$ is the rank of $\G$. \begin{dfn}
%	For any $m \in \N$ and  $z \in k^\times$ a primitive $m$th root of unity, we let $0 \leq l \leq m-1$ be the unique integer such that $\Psi(\psi(z)) = \exp^{\frac{2\pi i l}{m}}$. Let $z_n \defeq \psi^{-1}(\Psi^{-1}(\exp^{\frac{2\pi i l}{mn}}))$ be a primitive $n$th root of $z$. For any $t \in \T$, let $t_n \defeq \beta^{-1}((\beta(t))_n).$
%\end{dfn} 
%By the previous discussion,
%
%\begin{lem}\label{lem_isoQl} For any $t \in \T$ an element of order $m$, and any Kummer local system $\Ll = \lambda^*\left(\mathcal{E}_{n,\psi}\right)$, there exists an isomorphism $\nu_{\lambda,t} \defeq \lambda^*\left(\nu_{\lambda(t_n),n}\right)$ between $t^*\Ll$ and $\Ll$.
%\end{lem}
%\begin{lem}\label{lem_isostalks}
%	Let $m,n \in \N$ and $t \in \T$ an element of order $m$. Let $\Ll = \lambda^*\left(\Ee_{n,\psi}\right)$. The isomorphisms $\left(\nu_{\lambda,t}\right)_1: \left(\mathcal{E}_{n,\psi}\right)_{\lambda(t_n)} \to \left(\mathcal{E}_{n,\psi}\right)_1$ and $\eta_1 \circ \iota_{\lambda(t)}$ differ by multiplication by $\psi(\lambda(t_n))$.
%	In particular, for each  $s \in Z(\G)$ and $w \in W_\Ll$, writing $\lambda^w =\lambda\lambda_w^n$ for some $\lambda_w \in X(\T)$, $$\left(\nu_{\lambda^w,s}\right)_1 = \psi(\lambda_w(s))\left(\nu_{\lambda,s}\right)_1.$$
%\end{lem}
%
%\begin{proof} Let $\nu$ be as in Lemma \ref{lem_isoQl}. Observe that for any $z \in \k^\times$ a $m$th root of unity, \[\iota \circ \nu_{z,n} = \nu_{z,nm} \circ (z^n)^*(\iota)\] and that $\eta_1\circ \iota_1$ is the identity on $\left(\mathcal{E}_{n,\psi}\right)_1$. Thus, we can rewrite $\left(\nu_{\lambda,t}\right)_1 $ as 
%	\[\left(\nu_{\lambda,t}\right)_1 = \left(\nu_{\lambda(t_n),n}\right)_1 = \eta_1 \circ (\nu_{\lambda(t_n),nm})_1 \circ \iota_{\lambda(t_n)^n} =  \eta_1 \circ (\nu_{\lambda(t_n),nm})_1 \circ \iota_{\lambda(t)}.\]
%	We consider the image of any $v \in \left(\mathcal{E}_{n,\psi}\right)_1$ by $\left(\nu_{\lambda,t}\right)_1$. Then, we see that \begin{equation*}
%		\left(\nu_{\lambda,t}\right)_1(v) = \eta_1 \circ (\nu_{\lambda(t_n),nm})_1(\iota_{\lambda(t)}(v)) = \eta_1(\psi(\lambda(t_n))\iota_{\lambda(t)}(v))= \psi(\lambda(t_n))\eta_1(\iota_{\lambda(t)}(v)).
%	\end{equation*}
%	The second statement follows from the fact that $\lambda^w(s) = \lambda(s)$ since $s \in Z(\G)$.	
%\end{proof}
%
%
%%We now restrict ourselves to the case where $z$ is a primitive $m$th root of unity. We fix a field isomorphism $\Psi: \Ql \to \C$. \begin{dfn}
%%	For any $m \in \N$ and  $z \in k^\times$ a primitive $m$th root of unity, we let $0 \leq l \leq m-1$ be the unique integer such that $\Psi(\psi(z)) = \exp^{\frac{2\pi i l}{m}}$. Let $z_n \defeq \psi^{-1}(\Psi^{-1}(\exp^{\frac{2\pi i l}{mn}}))$ be a primitive $n$th root of $z$.
%%\end{dfn} 
%%By the previous discussion,
%%
%%\begin{lem}\label{lem_isoQl} For any $z \in k^\times$ a primitive $m$th root of unity, there exists an isomorphism $\nu \defeq \nu_{z_n,n}$ between $z^*\left(\left(\rho_n\right)_*\Ql\right)$ and $\left(\rho_n\right)_*\Ql$ which commutes with the action of $\mu_n$.
%%\end{lem}
%% We set a natural morphism on the stalks, given by the definition of the pushforward and of the stalks as direct limit:
%%\[\eta_1: \left(\left(\rho_{nm}\right)_*\Ql\right)_{1} \to \left(\left(\rho_{n}\right)_*\Ql\right)_{1} \] The morphism $\eta_1$ is given by projection on the coordinates which are $n$th roots of unity. It commutes with the action of $\mu_n$. Observe that $\eta_1\left(\left(\mathcal{E}_{nm,\psi}\right)_1\right) = \left(\mathcal{E}_{n,\psi}\right)_1$ and therefore $\eta_1$ defines an isomorphism from $\left(\mathcal{E}_{nm,\psi}\right)_1$ to $\left(\mathcal{E}_{n,\psi}\right)_1$ as $\mu_n$-modules. 
%%\begin{proof}
%%	We fix an isomorphism $\nu_0: \Ql \to z_n^*\Ql$, which we can assume is simply the identity on the stalks. From it, we get an isomorphism $$\nu \defeq (\rho_n)_*(\nu_0): \left(\left(\rho_n\right)_*\Ql\right) \to \left(\rho_n\right)_*z_n^*\left(\Ql\right)= z^*\left(\left(\rho_n\right)_*\Ql\right),$$ which commutes with the action of $\mu_n$.\\
%%	The isomorphism $\nu$ acts on the stalks simply by permuting the coordinates: sending the coordinate $x \in \mu^c_n$ to $z_nx \in \mu^{zc}_n$. 
%%\end{proof} 
%%\begin{enumerate}
%%	\item \[\nu_{z,n}: (z^n)^*\left(\rho_n\right)_*\Ql \to \left(\rho_n\right)_*z^*\Ql \to \left(\rho_n\right)_*z^*z_*\Ql \to \left(\rho_n\right)_*\Ql,\]
%%	where the first arrow is given by the change of basis, the second one by the fact that $z_*\Ql$ is in fact the constant sheaf and the last one by adjunction. \\
%%	In particular, the action of $\mu_n$ on $\left(\rho_n\right)_*\Ql$ is given by the maps $\nu_z$ for $z \in \mu_n$.
%%	\item \[\eta: \left(\rho_{nm}\right)_*\Ql \to  \]
%%	\item \[\iota: \left(\rho_{n}\right)_*\Ql \to \left(\rho_{nm}\right)_*\left(\rho_{m}\right)^* \Ql \to \left(\rho_{nm}\right)_*\Ql, \]
%%	where the first arrow is given by adjunction and the second by the fact that $\left(\rho_{m}\right)^* \Ql$ is the constant sheaf. 
%%
%%\end{enumerate}
%%
%%We fix two other natural isomorphisms:
%
%
%%We unfold the definition of $\mathcal{E}_{n,\psi}$ by focusing on the stalks. We fix $n \in \N$ and $c \in k^\times$ and define \[\mu_n^c \defeq \{x \in {k}^\times \mid x^n = c\}.\]  
%%The stalk $\left(\left(\rho_n\right)_*\Ql\right)_c$ can be seen as an $n$-dimensional $\Ql$-vector space, with coordinates indexed by $\mu_n^c$, and on which $\mu_n$ acts by permuting the coordinates. In other words, the action of $\mu_n$ on $\left(\left(\rho_n\right)_*\Ql\right)_c$ is induced by $\mu_n \times \mu_n^c \to \mu_n^c$, $\left(x,y\right) \mapsto xy$. 
%%In that setting, $\left(\mathcal{E}_{n,\psi}\right)_c$ is a $\Ql$-vector space of dimension one on which the action of $x \in \mu_n$ is simply multiplication by $\psi(x)$. 
%
%%By definition of the stalks as direct limit and of the pushforward, there exists a unique morphism $\eta^{c,n}_1: \left(\left(\rho_n\right)_*\Ql\right)_{c^n} \to \left(\Ql\right)_{c}$ for any $c \in k^\times$.
%%For any $m \in \N$ and $z \in k$ a primitive $m$th root of unity, we extend notation and define $\eta_1$ the unique morphism between $\left(\left(\rho_{nm}\right)_*\Ql\right)_{1}$ and $\left(\left(\rho_{n}\right)_*\Ql\right)_{1}$ and $\eta_z$ the unique morphism between $\left(\left(\rho_{nm}\right)_*\Ql\right)_{1}$ and $\left(\left(\rho_{n}\right)_*\Ql\right)_{z}$. The morphism $\eta_1$ (resp. $\eta_z$) is given by projection on the coordinates which are $n$th roots of unity (resp. $n$th roots of $z$). Both morphisms commute with the action of $\mu_n$. 
%%We also consider $\iota_1: \left(\left(\rho_{n}\right)_*\Ql\right)_{1} \to \left(\left(\rho_{nm}\right)_*\Ql\right)_{1}$ the inclusion morphism such that $\eta_1 \circ \iota_1$ is the identity. It also commutes with the action of $\mu_n$.\\
%%Observe that $\eta_1\left(\left(\mathcal{E}_{nm,\psi}\right)_1\right) = \left(\mathcal{E}_{n,\psi}\right)_1$ and therefore $\eta_1$ defines an isomorphism from $\left(\mathcal{E}_{nm,\psi}\right)_1$ to $\left(\mathcal{E}_{n,\psi}\right)_1$ as $\mu_n$-modules. Similarly, so does $\eta_z$ between $\left(\mathcal{E}_{nm,\psi}\right)_1$ and $\left(\mathcal{E}_{n,\psi}\right)_z$. \\
%%Therefore, we canonically identify $\left(\mathcal{E}_{n,\psi}\right)_1$ and $\left(\mathcal{E}_{n,\psi}\right)_z$ via $v \in \left(\mathcal{E}_{n,\psi}\right)_1$ corresponding to $\eta_z(\eta_1^{-1}(v)) =  \eta_z(\iota_1(v))\in \left(\mathcal{E}_{n,\psi}\right)_z$.\\
%
%
%%We fix a field isomorphism $\Psi: \Ql \to \C$. \begin{dfn}
%%	For any $m \in \N$ and  $z \in k^\times$ a primitive $m$th root of unity, we let $0 \leq l \leq m-1$ be the unique integer such that $\Psi(\psi(z)) = \exp^{\frac{2\pi i l}{m}}$. Let $z_n \defeq \psi^{-1}(\Psi^{-1}(\exp^{\frac{2\pi i l}{mn}}))$ be a primitive $n$th root of $z$.
%%\end{dfn} 
%%
%%\begin{lem}\label{lem_isoQl} For any $z \in k^\times$ a primitive $m$th root of unity, there exists an isomorphism $\nu$ between $\left(\left(\rho_n\right)_*\Ql\right)$ and $z^*\left(\left(\rho_n\right)_*\Ql\right)$ which commutes with the action of $\mu_n$, and which acts on the stalks by permuting coordinates. 
%%\end{lem}
%%\begin{proof}
%%	We fix an isomorphism $\nu_0: \Ql \to z_n^*\Ql$, which we can assume is simply the identity on the stalks. From it, we get an isomorphism $$\nu \defeq (\rho_n)_*(\nu_0): \left(\left(\rho_n\right)_*\Ql\right) \to \left(\rho_n\right)_*z_n^*\left(\Ql\right)= z^*\left(\left(\rho_n\right)_*\Ql\right),$$ which commutes with the action of $\mu_n$.\\
%%	The isomorphism $\nu$ acts on the stalks simply by permuting the coordinates: sending the coordinate $x \in \mu^c_n$ to $z_nx \in \mu^{zc}_n$. 
%%\end{proof}
%
%%\begin{rmk}
%%\end{rmk}
%
%
%
%%\begin{lem}\label{lem_isostalks}
%%	Let $m,n \in \N$ and $z \in k^\times$ a primitive $m$th root of unity. The isomorphisms $\nu_1: \left(\mathcal{E}_{n,\psi}\right)_{z_n} \to \left(\mathcal{E}_{n,\psi}\right)_1$ and $\eta_1 \circ \iota_z$ differ by multiplication by $\psi(z_n)$.
%%\end{lem}
%%
%%\begin{proof} Let $\nu$ be as in Lemma \ref{lem_isoQl}. Observe that \[\iota \circ \nu_{z_n,n} = \nu_{z_n,nm} \circ z^*(\iota)\] and that $\eta_1\circ \iota_1$ is the identity on $\left(\mathcal{E}_{n,\psi}\right)_1$. Thus, we can rewrite $\nu_1$ as 
%%	\[\nu_1 = \eta_1 \circ (\nu_{z_n,nm})_1 \circ \iota_z.\]
%%	We consider the image of any $v \in \left(\mathcal{E}_{n,\psi}\right)_1$ by $\nu_1$. Then, we see that \begin{equation*}
%%		\nu(v) = \eta_1 \circ (\nu_{z_n,nm})_1(\iota_z(v)) = \eta_1(\psi(z_n)\iota_z(v))= \psi(z_n)\eta_1(\iota_z(v)).\qedhere
%%	\end{equation*}
%%\end{proof}
%
%\begin{lem}\label{lem_transphiLl}
%Let $z \in Z(\G)$, $w \in W_{\Ll}$, then there is $\lambda_w \in \Hom(\T, k^\times)$ depending on $\Ll$ such that
%$$\psi(\lambda_w(z))z^*(\phi^{{\Ll}}_w) = \phi^{z^*{\Ll}}_w \quad \text{ and } \,  \psi(\lambda_w(z))z^*(\tilde{\phi}^{{\Ll}}_w) = \tilde{\phi}^{z^*{\Ll}}_w.$$ 
%\end{lem}
%\begin{proof} We have $W_{z^*{\Ll}} = W_{{\Ll}}$ and $\phi^{z^*{\Ll}}_w$ is well-defined. 
%	Since $z^*(\phi^{{\Ll}}_w) \in \mathcal{H}_{z^*{\Ll},w}$, the two isomorphisms $z^*(\phi^{{\Ll}}_w)$ and $\phi^{z^*{\Ll}}_w$ differ by a scalar. To determine it, it suffices to consider the stalks at $1$. Recall that there is $\lambda_w \in \Hom(\T, k^\times)$ such that $\ad(w^{-1})^*{\Ll} \cong (\lambda_w^n\lambda)^*\mathcal{E}_{n,\psi}$.  We make a few remarks. Firstly, for any $\lambda,\mu \in \mathcal{S}(\T)$, we have $(\lambda\mu)^*\Ee_{n,\psi} = \lambda^*\Ee_{n,\psi} \otimes \mu^*\Ee_{n,\psi}$. Moreover, the adjunction map $\xi: (\rho_n)^*(\rho_{n})_*\Ql\to\Ql$ induces a morphism $\xi: (\lambda^n)^*(\rho_{n})_*\Ql \to \left(\lambda \circ \rho_n\right)^*(\rho_{n})_*\Ql \to \lambda^*\Ql \to \Ql$, which restrict to an isomorphism $(\lambda^n)^*\Ee_{n,\psi} \to \Ql$. Lastly, for any $t \in \T$, by naturality of $\nu_{\lambda(t),n}$ and $\xi$, we can check that the following diagram commute: \vspace{-3mm}\begin{center}
%		\begin{tikzcd}
%			t^*(\lambda^n)^*(\rho_{n})_*\Ql \arrow[rr, "t^*\lambda^*\xi"] \arrow[d, "(\lambda^n)^*\left(\nu_{\lambda(t),n}\right)"'] &  & t^*{\lambda^*\Ql}\arrow[d, "\lambda^*\nu_{\lambda(t),1}"]    \\
%			(\lambda^n)^*(\rho_{n})_*\Ql  \arrow[rr, "\lambda^*\xi"']                                                 &  & {\lambda^*\Ql}
%		\end{tikzcd} 
%	\end{center}
%	Therefore the first two observations leads to the the following commutative diagram: \begin{center}
%		\begin{tikzcd}
%			t^*(\lambda^n\mu)^*\Ee_{n,\psi} = t^*(\lambda^n)^*\Ee_{n,\psi} \otimes t^*\mu^*\Ee_{n,\psi} \arrow[rr, "t^*\lambda^*\xi \otimes id"] \arrow[d, "(\lambda^n)^*\left(\nu_{\lambda(t),n}\right) \otimes \mu^*\left(\nu_{\mu(t_n),n}\right)"'] &  & t^*{\lambda^*\Ql} \otimes t^*\mu^*\Ee_{n,\psi}\arrow[d, "\lambda^*\nu_{\lambda(t),1} \otimes \mu^*\left(\nu_{\mu(t_n),n}\right)"]    \\
%			(\lambda^n\mu)^*\Ee_{n,\psi} = (\lambda^n)^*\Ee_{n,\psi} \otimes \mu^*\Ee_{n,\psi}  \arrow[rr, "\lambda^*\xi \otimes id"']                                                 &  & {\lambda^*\Ql} \otimes \mu^*\Ee_{n,\psi} 
%		\end{tikzcd} 
%	\end{center}
%We conclude that this last diagram commutes as well, since $\phi^\Ll_w$ is a multiple of $\lambda_w^*\xi \otimes id:$ \begin{center}
%	\begin{tikzcd}
%		z^*\ad(w^{-1})^*{\Ll} \arrow[rr, "z^*\phi_w^{\Ll}"] \arrow[d, "\nu_{\lambda^w,z}"'] &  & z^*{\Ll}\arrow[d, "\nu_{\lambda,z}"]    \\
%		\ad(w^{-1})^*{\Ll}  \arrow[rr, "\phi^{\Ll}_w"']                                                 &  & {\Ll}
%	\end{tikzcd} 
%\end{center}
%Taking the stalks at $1$ (recall that $\left(\phi^{\Ll}_w\right)_1$ is the identity) and applying Lemma \ref{lem_isostalks}, we conclude that  $(z^*\phi^{{\Ll}}_w)_1$ is simply multiplication by $ \psi(\lambda_w(z))^{-1},$ whence $\psi(\lambda_w(z))z^*(\phi^{{\Ll}}_w) = \phi^{z^*{\Ll}}_w$ and $\psi(\lambda_w(z))z^*(\tilde{\phi}^{{\Ll}}_w) = \tilde{\phi}^{z^*{\Ll}}_w$. 
%%\begin{equation*}
%%		\psi(\lambda_w(z))z^*(\phi^{{\Ll}}_w) = \phi^{z^*{\Ll}}_w \text{ and } \psi(\lambda_w(z))z^*(\tilde{\phi}^{{\Ll}}_w) = \tilde{\phi}^{z^*{\Ll}}_w. \qedhere
%%		\end{equation*}  
%\end{proof}
%
%

%
%Observe that thanks to Lemma \ref{lem_isoQl}, we have an isomorphism $\nu_{\lambda,t}:  z^*\Ll = \lambda^*{\lambda(z)}^*\mathcal{E}_{n,\psi} \to \Ll .$  In particular, 
%the following diagram commutes:
%\begin{center}
%	\begin{tikzcd}
%	z^*\ad(w^{-1})^*{\Ll} = \ad(w^{-1})^*z^*{\Ll} \arrow[rr, "z^*\phi_w^{\Ll}"] \arrow[d, "\nu"'] &  & z^*{\Ll}\arrow[d, "\nu"]    \\
%		\ad(w^{-1})^*{\Ll}  \arrow[rr, "\phi^{\Ll}_w"']                                                 &  & {\Ll}
%	\end{tikzcd} 
%\end{center}
%%
%Therefore, the isomorphism $\nu$ induces an isomorphism, $z^*K \cong IC(\T,z^*( \Ll))[\dim \T] \cong K$. However, we might not have an isomorphism between $\left(A_E^\Ll\right)$ and $A_E^{z^*\Ll}$ for $E \in \irr(W_\Ll)$. 

%\begin{lem}\label{lem_transphiLl2}
%	Let $z \in Z(\G)$, $w \in W_{\Ll}$, then there is $\lambda_w \in \Hom(\T, k^\times)$ depending on $\Ll$ such that
%	$$\psi(\lambda_w(z))z^*(\phi^{{\Ll}}_w) = \phi^{z^*{\Ll}}_w \quad \text{ and } \,  \psi(\lambda_w(z))z^*(\tilde{\phi}^{{\Ll}}_w) = \tilde{\phi}^{z^*{\Ll}}_w.$$ 
%\end{lem}
%\begin{proof}
%	We have $W_{z^*{\Ll}} = W_{{\Ll}}$ and $\phi^{z^*{\Ll}}_w$ is well-defined. 
%	Since $z^*(\phi^{{\Ll}}_w) \in \mathcal{H}_{z^*{\Ll},w}$, the two isomorphisms $z^*(\phi^{{\Ll}}_w)$ and $\phi^{z^*{\Ll}}_w$ differ by a scalar. To determine it, it suffices to consider the stalks at $1$. Recall that there is $\lambda_w \in \Hom(\T, k^\times)$ such that $\ad(w^{-1})^*{\Ll} \cong (\lambda_w^n\lambda)^*\mathcal{E}_{n,\psi}$. We write $\lambda' \defeq \lambda^w = \lambda_w^n\lambda$. Passing from  ${\Ll}_z = \left(z^*\Ll\right)_1$ to ${\Ll}_1$ is given by the isomorphism $\nu_1$. Let $m$ be the order of $z$. By Lemma \ref{lem_isostalks}, $\nu_1 = \eta_1 \circ (\nu_{\lambda(z)_n,nm})_1 \circ \iota_z$. We have the following diagram:
%	\begin{center}
%		\begin{tikzcd}
%			\left(\Ee_{n,\psi}\right)_1 = \left(\ad(w^{-1})^*{\Ll}\right)_1 \arrow[rr, "(\phi_w^{\Ll})_1 = id"] \arrow[d, "\iota_1"'] &  & {\Ll}_1 = \left(\Ee_{n,\psi}\right)_1 \arrow[d, " \iota_1"]    \\
%			\left(\Ee_{nm,\psi}\right)_1 \arrow[rr, "id"] \arrow[d, "a_{\lambda'(z)_n}"'] &  &  \left(\Ee_{nm,\psi}\right)_1 \arrow[d, "a_{\lambda(z)_n}"]    \\
%			\left(\Ee_{nm,\psi}\right)_1  \arrow[rr, "a_{\lambda_w(z)^{-1}} = \dot \psi(\lambda_w(z)^{-1})"] \arrow[d, "\eta_{\lambda'(z)}"'] &  &  \left(\Ee_{nm,\psi}\right)_1 \arrow[d, "\eta_{\lambda(z)}"]    \\
%			\left(\Ee_{n,\psi}\right)_{\lambda'(z)} =\left(\ad(w^{-1})^*{\Ll}\right)_z \arrow[rr, "(z^*\phi^{z^*\Ll}_w)_1"']                                                 &  & {\Ll}_z = \left(\Ee_{n,\psi}\right)_{\lambda(z)}
%		\end{tikzcd} 
%	\end{center}
%		\begin{center}
%		\begin{tikzcd}
%		\left(\Ee_{n,\psi}\right)_{\lambda'(z)} =\left(\ad(w^{-1})^*{\Ll}\right)_z \arrow[rr, "(z^*\phi^{\Ll}_w)_1"] \arrow[d, "\iota_{\lambda'(z)}"'] &  & {\Ll}_z = \left(\Ee_{n,\psi}\right)_{\lambda(z)} \arrow[d, " \iota_{\lambda(z)}"]   \\
%			\left(\Ee_{nm,\psi}\right)_1 \arrow[rr, "(\nu_{\lambda_w(z)^{-1},nm})_1 = \dot \psi(\lambda_w(z)^{-1})"] \arrow[d, "(\nu_{\lambda'(z)_n,nm})_1"'] &  &  \left(\Ee_{nm,\psi}\right)_1 \arrow[d, "(\nu_{\lambda(z)_n,nm})_1"]    \\
%			\left(\Ee_{nm,\psi}\right)_1  \arrow[rr, "id"] \arrow[d, "\eta_{1}"'] &  &  \left(\Ee_{nm,\psi}\right)_1 \arrow[d, "\eta_{1}"]    \\
%				\left(\Ee_{n,\psi}\right)_1 = \left(\ad(w^{-1})^*{\Ll}\right)_1   \arrow[rr, "(\phi_w^{\Ll})_1 = id"']                                                &  & {\Ll}_1 = \left(\Ee_{n,\psi}\right)_1 
%		\end{tikzcd} 
%	\end{center}
%	The external diagram commutes and the bottom two squares as well by definition of the action of $\mu_{nm}$. Moreover, all the maps are isomorphisms, thus the first square commutes as well. It implies that  $(z^*\phi^{{\Ll}}_w)_1$ is simply multiplication by $ \psi(\lambda_w(z))^{-1}$ whence \begin{equation*}
%	\psi(\lambda_w(z))z^*(\phi^{{\Ll}}_w) = \phi^{z^*{\Ll}}_w \text{ and } \psi(\lambda_w(z))z^*(\tilde{\phi}^{{\Ll}}_w) = \tilde{\phi}^{z^*{\Ll}}_w. \qedhere
%	\end{equation*}  
%\end{proof}

\begin{rmk}
	Observe that the map $W_\Ll \to \Ql^\times, w \mapsto \psi(\lambda_w(z))$ is a group homomorphism since $z^*\phi^{{\Ll}}_{w'}\circ  \ad((\dot{w}')^{-1})^*z^*(\phi^{{\Ll}}_{w}) = z^*\left(\phi^{{\Ll}}_{w'}\circ  \ad((\dot{w}')^{-1})^*(\phi^{{\Ll}}_{w})\right) = z^*\phi^{{\Ll}}_{ww'}$ for all $w,w' \in W_\Ll.$ Thus, $\psi(\lambda_{w'}(z))^{-1} \circ \psi(\lambda_{w}(z))^{-1} = \psi(\lambda_{ww'}(z))^{-1}.$ 
\end{rmk}

We gather different facts on $\psi(\lambda_w(z))$ from \cite[$\S$ 11.8]{lusztigCharacterSheavesIII1985}:
\begin{lem}\label{lem_valchiz}
	Let $z \in Z(\G)$, ${\Ll} = \lambda^*(\mathcal{E}_{n,\psi})$. Then 
	\begin{enumerate}
		\item $\psi(\lambda_w(z)) = 1$ if $z \in Z^\circ(\G)$ or $w \in W^\circ_{\Ll}$,
		\item the map $W_{\Ll}/W^\circ_{\Ll} \to \Hom(Z(\G)/Z^\circ(\G), \, \Ql^\times)$, $w \mapsto \left(\bar{z} \to \psi(\lambda_w(z))\right)$ is injective. 
	\end{enumerate}
\end{lem}

\subsubsection{Translation of character sheaves} 
\begin{lem}\label{lem_translationCS}
	For $z \in Z(\G)$, $E \in \irr(W_{\Ll})$ we have 
	\[A^{{\Ll}}_E \cong A^{z^*{\Ll}}_{E\cdot \chi^z},\]
	where $\chi^z: W_{\Ll} \to \Ql^\times$ is given by $w \mapsto \psi(\lambda_w(z))$. 
\end{lem}

\begin{proof}	
	For $w \in W_{\Ll}$, we can define two embeddings of  $\mathcal{H}_{z^*{\Ll},w}$ into $\mathcal{H}_{\Ql,w}$: the first one being the usual one identifying $\phi^{z^*{\Ll}}_w$ with $\phi^{\Ql}_w$ and the second one identifying $z^*(\phi^{{\Ll}}_w)$ with $\phi^{\Ql}_w$. So we get two isomorphisms between $\Ql\left[ W_{\Ll}\right] $ and $ \End(IC(\G,\delta_*(\tilde{z^*{\Ll}}))).$ From Lemma \ref{lem_transphiLl}, we see that they differ by multiplication with $\psi(\lambda_w(z))$. We define $\chi^z: W_\Ll \to \Ql$ by $w \mapsto \psi(\lambda_w(z))$ for any $w \in W_\Ll$.  On one hand we have, 
	%Let's fix $E_0 \in \irr(\End(IC(\overline{Y_{\T}},\delta_*(\tilde{{\Ll}}))))$ such that it corresponds under the second isomorphism to $E_1 \in \irr(W_{\Ll})$ .
	\begin{align*}
		A^{{\Ll}}_E &\cong \Hom_{\End(IC(\G,\delta_*(\tilde{{\Ll}})))}\left(E, IC\left(\G,\delta_*(\tilde{{\Ll}})\right)\right)&\\
		&\cong \Hom_{W_{\Ll}}\left(E, IC\left(\G,\delta_*(\tilde{{\Ll}})\right)\right) \quad &(\phi^{{\Ll}}_w \leftrightarrow \phi^{\Ql}_w)\\
		& \cong z^*\Hom_{W_{\Ll}}(E,z^*IC(\G,\delta_*(\tilde{{\Ll}}))) \quad &(z^*\phi^{{\Ll}}_w \leftrightarrow \phi^{\Ql}_w) \\
		& \cong \Hom_{W_{\Ll}}(E,IC(\G,\delta_*(\tilde{z^*{\Ll}}))). &
	\end{align*}
	
	\noindent On the other hand, for $E' \in \irr(W_\Ll)$, we have 
	\begin{align*}
		A^{z^*{\Ll}}_{E'} &\cong z^*\Hom_{\End(IC(\G,\delta_*(\tilde{z^*{\Ll}})))}\left(E', IC\left(\G,\delta_*(\tilde{z^*{\Ll}})\right)\right)&\\
		&\cong \Hom_{W_{\Ll}}(E',IC(\G,\delta_*(\tilde{z^*{\Ll}})))  &(\phi^{z^*{\Ll}}_w = \chi^z(w)z^*\phi^{{\Ll}}_w \leftrightarrow \phi^{\Ql}_w)	\\
		&\cong \Hom_{W_{\Ll}}(E'\cdot (\chi^z)^{-1},IC(\G,\delta_*(\tilde{z^*{\Ll}}))).  &(z^*\phi^{{\Ll}}_w \leftrightarrow \phi^{\Ql}_w)	
	\end{align*}
	We conclude that $A^{{\Ll}}_E\cong A^{z^*{\Ll}}_{E'}$ if and only if $E' = E \cdot \chi^z.$
\end{proof}

==> counting.tex <==
Main reference: \cite[Section 2.2, Section 2.3]{chanebBasicSetsDecomposition2019}
\begin{res} 
Let $t \in \G^*$ be a semisimple element of order prime to $\ell$. Set\[ B_t(\G) = \bigsqcup \mathcal{E}(G,ts),\] where $s$ runs over the semisimple $\ell$-elements of $G^*$. Then $B_t(\G)$ is an union of $\ell$-blocks fo $\G$. 
\end{res}

If $t =1$, we call it the \textbf{unipotent blocsk}. 

\begin{dfn}
	Let $\Cc \in X_\G$ be a special class. 	
	We define the \textbf{ordinary canonical quotient} $\Omega_{\G,u}$ as the quotient of $A_\G(u)$ by the intersection of the kernels  of the $\psi \in \irr(A_\G(u))$ such that for some $\theta \in \irr(W)$, with $i_\G(\theta)= (\Cc,\psi)$ and the number $a_\theta$ is maximal (equal to $a_{\theta_1}$, where $i_\G(\theta_1)= (\Cc,1)$ is the special character).
\end{dfn}


\begin{dfn}
	Let $\Cc$ be an $\ell$-special class. Let $P$ be a projective indecomposable module of $kA_\G(u)$ and $\Psi$ its character. We define $a_\Psi$	
\[a_\Phi = \min \{a_\theta \mid \theta \in \irr(W), i_\G(\theta)= (\Cc,\psi), d_{\psi,\Psi} \neq 0 \} \]
We define the \textbf{$\ell$-canonical quotient} $\Omega^\ell_{\G,u}$ as the quotient of $A_\G(u)$ by intersection of the kernels of the projective indecomposable modules $P$ with $a_\Psi$ maximal.
\end{dfn}

\begin{id}
$a_\Phi$ is maximal if it is equal to the $a$ corresponding to the projective indecomposable module associated to the trivial one. 
\end{id}

\begin{id}
	If we add the condition that $\Omega_{C_{\textbf{G}^*}(s), v} \cong \Omega^\ell_{\G,u}$ in the definition of $\ell$-special, we obtain the same results.
\end{id}
\begin{proof}
	Checked by Julia.
\end{proof}

For $A$ a finite group, we define $\mathcal{M}(A)$ as the set of $A$-conjugacy classes of pairs $[a,\phi]$ with $a \in A$ and $\phi \in \irr(A)$. We also write $\mathcal{M}^\ell(A)$ for the set of $A$-conjugacy classes of pairs $[a,\phi]$ with $a \in A$ and $\phi \in \irr_k(A)$.

\begin{res}\label{nbunipmod}
	\begin{itemize}
			\item When $\ell$ is good, $\Omega^\ell_{\G,u} = \Omega_{\G,u}$.
			\item If $\G$ is simple adjoint of exceptional type, summing $|\mathcal{M}^\ell(\Omega^\ell_{\G,u})|$ over all $\ell$-special unipotent classes gives the number of indecomposable projective $k\G$-modules in the unipotent block.
	\end{itemize}
\end{res}

We write $\alpha_{\ell,u} \defeq |\mathcal{M}^\ell(\Omega^\ell_{\G,u})|$.

==> d7a5.tex <==
 \subsubsection{The unipotent conjugacy class $\Cc = E_7(a_5)$ when $\ell = 2$}
 
 In this case, maybe reduce to $C_{G^*}(s)$ ???\\
 
In this case there is $(s,v)$ satifies Property (P).
 In that case, we have $A_\G(u) = \Omega^2_{\G,u}\cong \Omega_{C_{\textbf{G}^*}(s), v} = A_{C_{\textbf{G}^*}(s)}(v) \cong S_3$
 So the value of the characteristic function of a character sheaf in $\hat{G}_{(s,v)}$  is known exactly on the unipotent support and should work in the proof in \cite[Proposition 8.8]{brunatUnitriangularShapeDecomposition2020}. By \cite[Cor 3.3]{geckUnipotentSupportCharacter2008a}, there should be $|\irr(A_\G(u))| = 3$ characters sheaves in $\hat{G}_{(s,v)}$  that have nonzero values on the unipotent support $\Cc^F$, (the ones indexed by $[1,\phi]$ $\phi \in \irr(A_\G(u))$?). All the other would have values zero on $\Cc^F$. We would need the values of the characteristic function of a character sheaf in $\hat{G}_{(s,v)}$ on any conjugacy class with unipotent part equal to the unipotent support. We would also need to check that for $\chi_{[a,\phi]}$ a characteristic function of a character sheaf in $\hat{G}_{(s,v)}$, we have $\chi_{[a,\phi]}(bu) = 0$  unless $b$ is conjugate to $a$ in $S_3$.


%\[[ [ ReflectionSubgroup(CoxeterGroup("E",8), [ 2, 3, 4, 5, 6, 7, 8, 97 ]), 2, 
%58, CoxeterGroup() ], \]
%\[[ ReflectionSubgroup(CoxeterGroup("E",8), [ 2, 3, 4, 5, 6, 7, 8, 97 ]), 2, 
%25, CoxeterGroup() ],\] 
%\[[ ReflectionSubgroup(CoxeterGroup("E",8), [ 1, 2, 4, 5, 6, 7, 8, 114 ]), 4, 
%3, CoxeterGroup() ], \]
%\[[ ReflectionSubgroup(CoxeterGroup("E",8), [ 1, 2, 3, 4, 5, 6, 7, 120 ]), 2, 
%57, CoxeterGroup("A",2) ] ]\]

==> e6a3-a1.tex <==
 \subsubsection{The $3$-special unipotent conjugacy class $\Cc = E_6(a_3) + A_1$ when $\ell = 3$}
 
 In this case, $A_\G(u)\cong \Omega^3_{\G,u} \cong S_2$. Using Chevie, we observe that there is $g =sv \in \G^*$ such that its image $\Phi(g)$ under Lusztig's map is $\Cc = E_6(a_3) + A_1$. Moreover, in that case, $\Omega_{C_{\G^*}(s),v} \cong S_2$.\\
 
 [ ReflectionSubgroup(CoxeterGroup("E",8), [ 1, 2, 3, 4, 5, 6, 8, 119 ]), 3, 
 49, CoxeterGroup("A",1) ] 
 \\
 

 We assume there exists an admissible covering $A$ such that $A \cong A_\G(u)$.
 Then we do the exact same construction of the Kawanaka characters as in the special case (definition \ref{dfn_Kawchar}.) We obtain four Kawanaka characters: $K^\G_{[1,1]},K^\G_{[1,\varepsilon]},K^\G_{[-1,1]},K^\G_{[-1,\varepsilon]}$. 

 Moreover \[\Gamma_{u_1} = K^\G_{[1,1]} + K^\G_{[1,\varepsilon]} \text{ and } \Gamma_{u_{-1}} = K^\G_{[-1,1]} + K^\G_{[-1,\varepsilon]}.\] 
 Notice that if $[a,\phi] \neq [b,\psi]$, then \[\langle \hat{K}_{[a,\phi]},\hat{K}_{[b,\psi]}\rangle = 0.\]
 
  The Fourier transform is given by
  \[\frac{1}{2}\begin{pmatrix}
  1 &1&1&1 \\
  1 &1&-1&-1 \\
  1 &-1&1&-1 \\
  1 &-1&-1&1
  \end{pmatrix}.\]
 
 Then we have \[\langle \hat{F}_{[a,\phi]},\hat{F}_{[a,\phi]}\rangle = 1,\]
 and \begin{align}\langle \hat{F}_{[1,1]},\hat{F}_{[1,\varepsilon]}\rangle &= \langle \hat{F}_{[-1,1]},\hat{F}_{[-1,\varepsilon]}\rangle\\ \langle \hat{F}_{[1,1]},\hat{F}_{[-1,1]}\rangle &= \langle \hat{F}_{[1,\varepsilon]},\hat{F}_{[-1,\varepsilon]}\rangle \\ \langle \hat{F}_{[1,1]},\hat{F}_{[-1,\varepsilon]}\rangle &= \langle \hat{F}_{[1,\varepsilon]},\hat{F}_{[-1,1]}\rangle.\end{align}
 
 Then on one hand \[\langle \hat{K^\G}_{[1,\varepsilon]},\hat{F}_{[-1,\varepsilon]}\rangle =-\frac{1}{2}\langle \hat{K^\G}_{[1,\varepsilon]},\hat{K^\G}_{[1,\varepsilon]}\rangle, \]
 but on the other hand,
 \begin{align*}
\langle \hat{K^\G}_{[1,\varepsilon]},\hat{F}_{[-1,\varepsilon]}\rangle &= \frac{1}{2}(\langle \hat{F}_{[1,1]},\hat{F}_{[-1,\varepsilon]}\rangle + \langle \hat{F}_{[1,\varepsilon]},\hat{F}_{[-1,\varepsilon]}\rangle  -\langle \hat{F}_{[-1,1]},\hat{F}_{[-1,\varepsilon]}\rangle -\langle \hat{F}_{[-1,\varepsilon]},\hat{F}_{[-1,\varepsilon]}\rangle)\\
& = \frac{1}{2}(\langle \hat{F}_{[1,\varepsilon]},\hat{F}_{[-1,1]}\rangle + \langle \hat{F}_{[1,\varepsilon]},\hat{F}_{[-1,\varepsilon]}\rangle - \langle \hat{F}_{[1,1]},\hat{F}_{[1,\varepsilon]}\rangle -\langle \hat{F}_{[1,\varepsilon]},\hat{F}_{[1,\varepsilon]}\rangle) \\
&=- \hat{F}_{[1,\varepsilon]},\hat{K^\G}_{[1,\varepsilon]}\rangle

 \end{align*}
 %\begin{align*}
% [ ReflectionSubgroup(CoxeterGroup("E",8), [ 1, 3, 4, 5, 6, 7, 8, 112 ]), 3, 
%4, CoxeterGroup() ], \\
%[ ReflectionSubgroup(CoxeterGroup("E",8), [ 1, 2, 3, 5, 6, 7, 8, 116 ]), 6, 
%12, CoxeterGroup() ], \\
%[ ReflectionSubgroup(CoxeterGroup("E",8), [ 1, 2, 3, 4, 5, 6, 8, 119 ]), 3, 
%49, CoxeterGroup("A",1) ] 
% \end{align*}

 

==> e6a3_a1_bis.tex <==
\subsubsection{General approach for the last cases}

We fix an $F$-stable unipotent class $\Cc$, an admissible covering $(A, \lambda)$ for $\Omega_{\G,\Cc}$ and a set $\{u_a \mid a\in A\}$ of admissible representatives. Let $g =sv =vs \in \G^*$ where $s\in (\G^*)^{F^*}$ semisimple and $v \in \G^*$ unipotent such that $\Phi(g) = \Cc$. \\

\begin{prop}
Suppose that there exists an $F$-stable character sheaf $\mathcal{A} \in \hat{\G}_s$ with unipotent support $\Cc$ such that for all $[b,\phi] \in \Mm(A)$ \[|\langle F^G_{[b,\phi]}, D_\G(\chi_\mathcal{A}) \rangle| = \begin{cases}
	x_\mathcal{A}  &\text{ if } [b,\phi] =[1,1] \\
	0 &\text{ otherwise,}
\end{cases}\]
for some $x_\mathcal{A} \in \C^\times$.
We assume as well that $A \cong \Omega_{\G,\Cc}$.\\
Then, the decomposition of the character $K^G_{[a,\phi]}$ into irreducible characters of $\G^F$ has at most one Alvis-Curtis dual of irreducible character in $\irr(\G^F)_g$ with unipotent support $\Cc$ and it occurs with multiplicity one. Furthermore, every irreducible character Alvis-Curtis dual of irreducible character in $\irr(\G^F)_g$ with unipotent support $\Cc$ occurs in exactly one $K^G_{[a,\phi]}$ for some $[a,\phi]\in \Mm(A)$.\\
\end{prop}
\begin{proof}
For $\theta$ a class function of $\G^F$, we denote by $\hat{\theta}$ the projection of $\theta$ on the space spanned by the Alvis-Curtis duals of irreducible characters in $\irr(\G^F)_g$ with unipotent support $\Cc$. It is equal to the set spanned by the Alvis-Curtis duals of the characteristic functions of the $F$-stable characters sheaves in $\hat{G}_s$ with unipotent support $\Cc$. We denote by $E$ the set of the $F$-stable characters sheaves in $\hat{G}_s$ with unipotent support $\Cc$.  \\
\todo{check it is true}
We fix $[a,\phi] \in \Mm(A)$. We have \begin{align*}
	K^G_{[a,\phi]} &= \sum_{[b,\psi] \in \Mm(A)} \{[a,\phi],[b,\psi]\}F^G_{[b,\psi]}\\
	&=  \{[a,\phi],[1,1]\}F^G_{[1,1]} + \sum_{[b,\psi] \in \Mm(A)\backslash{[1,1]}} \{[a,\phi],[b,\psi]\}F^G_{[b,\psi]}\\
	&= \frac{1}{|C_A(a)|}F^G_{[1,1]} + \sum_{[b,\psi] \in \Mm(A)\backslash\{[1,1]\}} \{[a,\phi],[b,\psi]\}F^G_{[b,\psi]}.
\end{align*}
Thus \[\hat{K}^G_{[a,\phi]} =  \frac{x_\mathcal{A}}{|C_A(a)|}D_\G(\chi_\mathcal{A}) + \sum_{\mathcal{A}' \in E\backslash\{A\}x_{\mathcal{A}'}^{[a,\phi]}}D_\G(\chi_{\mathcal{A}'}), \]
with $x_{\mathcal{A}'}^{[a,\phi]} \in \C$ for all $\mathcal{A}' \in E\backslash\{A\}$.\\
The Alvis-Curtis duals of the characteristic functions of character sheaves in $E$ is an orthonormal family. Therefore, we get \begin{align*}
	\langle \hat{K}^G_{[a,\phi]} , \hat{K}^G_{[a,\phi]}\rangle 
	&= \frac{|x_\mathcal{A}|^2}{|C_A(a)|^2} + \sum_{\mathcal{A}' \in E\backslash\{A\}}x_{\mathcal{A}'}^{[a,\phi]}\overline{x_{\mathcal{A}'}^{[a,\phi]}} > 0. 
\end{align*}
Now by construction, $\hat{K}^G_{[a,\phi]}$ is a character of $\G^F$, thus for all $[a,\phi], [b,\psi] \in \Mm(A) = \Mm(\Omega_{\G,\Cc})$, we have \[\langle \hat{K}^G_{[a,\phi]} , \hat{K}^G_{[a,\phi]}\rangle  \geq 1, \]
and  \[\langle \hat{K}^G_{[a,\phi]} , \hat{K}^G_{[b,\psi]}\rangle  \geq 0. \]
By the decomposition of GGGC into Kawanaka characters (\ref{KawGGGr}), we get for all $a \in A$, 
\[\langle \hat{\Gamma}_{u_a}, \hat{\Gamma}_{u_a}\rangle \geq \sum_{\phi \in \irr(C_A(a))}\phi(1)^2\langle \hat{K}^G_{[a,\phi]} , \hat{K}^G_{[a,\phi]}\rangle \geq \sum_{\phi \in \irr(C_A(a))}\phi(1)^2.\]
On the other hand, by \cite[Rmk 4.4]{geckUnipotentSupportCharacter2008a},\todo{proof clear at least for $S_2$ and $S_3$ \cite[Prop 6.7]{hezardSupportUnipotentFaisceauxcaracteres2004}.} we have that 
\[\langle \hat{\Gamma}_{u_a}, \hat{\Gamma}_{u_a}\rangle = \sum_{\phi \in \irr(C_A(a))}\phi(1)^2\]

Consequently, we have that for all $[a,\phi] \neq [b,\psi] \in \Mm(A) = \Mm(\Omega_{\G,\Cc})$,  \[\langle \hat{K}^G_{[a,\phi]} , \hat{K}^G_{[a,\phi]}\rangle  = 1, \]
and  \[\langle \hat{K}^G_{[a,\phi]} , \hat{K}^G_{[b,\psi]}\rangle  = 0. \]
Since by assumption, we have that $F$ acts trivially on $\Omega_{\G,\Cc}$, there are exactly $Mm(\Omega_{\G,\Cc})$ irreducible characters of $\G^F$ with wave front set $\Cc$. 
\end{proof} 

\begin{rmk}
Observe that in this case, we obtain a similar result that in \ref{excellent}. 
\end{rmk}

\begin{rmk}
The condition in 
\end{rmk}

\paragraph{The unipotent conjugacy class $\Cc = E_6(a_3) + A_1$ when $\ell = 3$\\} 
We fix the setting in the case where the $F$-stable unipotent class is $\Cc = E_6(a_3) + A_1$ and $\ell =3$. We choose $s \in \T_0^*$ such that $C_{\G^*}(s)$ is of type $E_6 \times A_2$ and $v$ is the unipotent class of $E_6 \times A_2$ named $A2, 111$. 

Following \cite[$\S$ 10.2]{brunatUnitriangularShapeDecomposition2020} and 
we can choose $A = \langle \sigma \rangle$ with $\sigma$ is an isolated involution (hence $F$-stable) such that $C_\G^\circ(\sigma)$ is of type .
Using the example in my other notes, we see that . 

%&= \langle \frac{1}{|C_A(a)|}D_\G(\chi_\mathcal{A})\zeta + \sum_{\mathcal{A}' \in E\backslash\{A\}}x_{\mathcal{A}'}^{[a,\phi]}D_\G(\chi_{\mathcal{A}'}), \frac{1}{|C_A(a)|}D_\G(\chi_\mathcal{A})\zeta + \sum_{\mathcal{A}' \in E\backslash\{A\}}x_{\mathcal{A}'}^{[a,\phi]}D_\G(\chi_{\mathcal{A}'})\rangle\\
% 
% \subsubsection{The unipotent conjugacy class $\Cc = E_6(a_3) + A_1$ when $\ell = 3$}
% 
%
%Observe that the Fourier transformation is an involution. 
%Thus
%\begin{align*}
%	\langle \hat{K}_{[1,1]}, \hat{K}_{[1,1]} \rangle &= \frac{1}{4}\left( \langle \hat{F}_{[1,1]}, \hat{F}_{[1,1]} \rangle + \langle \hat{F}_{[1,1]}, \hat{F}_{[1,\varepsilon]} \rangle +\langle \hat{F}_{[1,1]}, \hat{F}_{[-1,1]} \rangle +\langle \hat{F}_{[1,1]}, \hat{F}_{[-1,\varepsilon]} \rangle\right)
%\\ 
%& + \frac{1}{4}\left(\langle \hat{F}_{[1,\varepsilon]}, \hat{F}_{[1,1]} \rangle +\langle \hat{F}_{[1,\varepsilon]}, \hat{F}_{[1,\varepsilon]} \rangle +\langle \hat{F}_{[1,\varepsilon]}, \hat{F}_{[-1,1]} \rangle+\langle \hat{F}_{[\varepsilon,1]}, \hat{F}_{[-1,\varepsilon]} \rangle\right)\\
%&+\frac{1}{4}\left(\langle \hat{F}_{[-1,1]}, \hat{F}_{[1,1]} \rangle + \langle \hat{F}_{[-1,1]}, \hat{F}_{[1,\varepsilon]} \rangle + \langle \hat{F}_{[-1,1]}, \hat{F}_{[-1,1]} \rangle + \langle \hat{F}_{[-1,1]}, \hat{F}_{[-1,\varepsilon]} \rangle\right)\\
%&+\frac{1}{4}\left(\langle \hat{F}_{[-1,\varepsilon]}, \hat{F}_{[1,1]} \rangle + \langle \hat{F}_{[-1,\varepsilon]}, \hat{F}_{[1,\varepsilon]} \rangle + \langle \hat{F}_{[-1,\varepsilon]}, \hat{F}_{[-1,1]} \rangle + \langle \hat{F}_{[-1,\varepsilon]}, \hat{F}_{[-1,\varepsilon]} \rangle \right)\\
%& = \frac{1}{4}\left(4 + 4\langle \hat{F}_{[1,1]}, \hat{F}_{[1,\varepsilon]} \rangle + 4\langle \hat{F}_{[1,1]}, \hat{F}_{[-1,1]} \rangle + 4\langle \hat{F}_{[1,1]}, \hat{F}_{[-1,\varepsilon]} \rangle \right)\\
%&= 1 +  \langle \hat{F}_{[1,1]}, \hat{F}_{[-1,1]} \rangle + \langle \hat{F}_{[1,1]}, \hat{F}_{[-1,\varepsilon]} \rangle\\
%&= 1 + \frac{1}{4}\left(3\langle \hat{K}_{[1,1]}, \hat{K}_{[1,1]} \rangle - \langle \hat{K}_{[1,\varepsilon]}, \hat{K}_{[1,\varepsilon]} \rangle -\langle \hat{K}_{[-1,1]}, \hat{K}_{[-1,1]} \rangle - \langle \hat{K}_{[-1,\varepsilon]}, \hat{K}_{[-1,\varepsilon]} \rangle\right)
%\end{align*}
%and 
%\begin{align*}
%	\langle \hat{K}_{[1,\varepsilon]}, \hat{K}_{[1,\varepsilon]} \rangle &= \frac{1}{4}\left( \langle \hat{F}_{[1,1]}, \hat{F}_{[1,1]} \rangle + \langle \hat{F}_{[1,1]}, \hat{F}_{[1,\varepsilon]} \rangle -\langle \hat{F}_{[1,1]}, \hat{F}_{[-1,1]} \rangle -\langle \hat{F}_{[1,1]}, \hat{F}_{[-1,\varepsilon]} \rangle\right)
%	\\ 
%	& + \frac{1}{4}\left(\langle \hat{F}_{[1,\varepsilon]}, \hat{F}_{[1,1]} \rangle +\langle \hat{F}_{[1,\varepsilon]}, \hat{F}_{[1,\varepsilon]} \rangle -\langle \hat{F}_{[1,\varepsilon]}, \hat{F}_{[-1,1]} \rangle-\langle \hat{F}_{[\varepsilon,1]}, \hat{F}_{[-1,\varepsilon]} \rangle\right)\\
%	&+\frac{1}{4}\left(-\langle \hat{F}_{[-1,1]}, \hat{F}_{[1,1]} \rangle - \langle \hat{F}_{[-1,1]}, \hat{F}_{[1,\varepsilon]} \rangle + \langle \hat{F}_{[-1,1]}, \hat{F}_{[-1,1]} \rangle + \langle \hat{F}_{[-1,1]}, \hat{F}_{[-1,\varepsilon]} \rangle\right)\\
%	&+\frac{1}{4}\left(-\langle \hat{F}_{[-1,\varepsilon]}, \hat{F}_{[1,1]} \rangle - \langle \hat{F}_{[-1,\varepsilon]}, \hat{F}_{[1,\varepsilon]} \rangle + \langle \hat{F}_{[-1,\varepsilon]}, \hat{F}_{[-1,1]} \rangle + \langle \hat{F}_{[-1,\varepsilon]}, \hat{F}_{[-1,\varepsilon]} \rangle \right)\\
%	& = \frac{1}{4}\left(4 + 4\langle \hat{F}_{[1,1]}, \hat{F}_{[1,\varepsilon]} \rangle - 4\langle \hat{F}_{[1,1]}, \hat{F}_{[-1,1]} \rangle - 4\langle \hat{F}_{[1,1]}, \hat{F}_{[-1,\varepsilon]} \rangle \right)\\
%	&= 1 +  \frac{1}{4}\left( - \langle \hat{K}_{[1,1]}, \hat{K}_{[1,1]} \rangle + 3\langle \hat{K}_{[1,\varepsilon]}, \hat{K}_{[1,\varepsilon]} \rangle -\langle \hat{K}_{[-1,1]}, \hat{K}_{[-1,1]} \rangle - \langle \hat{K}_{[-1,\varepsilon]}, \hat{K}_{[-1,\varepsilon]} \rangle\right),\end{align*}
%
%Thus, we obtain \[2\langle \hat{K}_{[1,1]}, \hat{K}_{[1,1]} \rangle - \langle \hat{K}_{[1,\varepsilon]}, \hat{K}_{[1,\varepsilon]} \rangle = - \langle \hat{K}_{[1,1]}, \hat{K}_{[1,1]} \rangle + 2\langle \hat{K}_{[1,\varepsilon]}, \hat{K}_{[1,\varepsilon]} \rangle. \]
%
%Since $1 \leq \langle \hat{K}_{[1,1]}, \hat{K}_{[1,1]} \rangle + \langle \hat{K}_{[1,\varepsilon]}, \hat{K}_{[1,\varepsilon]} \rangle \leq 3$, we then must have
%\[\langle \hat{K}_{[1,1]}, \hat{K}_{[1,1]} \rangle = \langle \hat{K}_{[1,\varepsilon]}, \hat{K}_{[1,\varepsilon]} \rangle = 1.\]
%
%Now we also have \begin{align*}
%	\langle \hat{K}_{[-1,1]}, \hat{K}_{[-1,1]} \rangle &= \frac{1}{4}\left( \langle \hat{F}_{[1,1]}, \hat{F}_{[1,1]} \rangle - \langle \hat{F}_{[1,1]}, \hat{F}_{[1,\varepsilon]} \rangle +\langle \hat{F}_{[1,1]}, \hat{F}_{[-1,1]} \rangle -\langle \hat{F}_{[1,1]}, \hat{F}_{[-1,\varepsilon]} \rangle\right)
%	\\ 
%	&  \frac{1}{4}\left(-\langle \hat{F}_{[1,\varepsilon]}, \hat{F}_{[1,1]} \rangle +\langle \hat{F}_{[1,\varepsilon]}, \hat{F}_{[1,\varepsilon]} \rangle -\langle \hat{F}_{[1,\varepsilon]}, \hat{F}_{[-1,1]} \rangle+\langle \hat{F}_{[\varepsilon,1]}, \hat{F}_{[-1,\varepsilon]} \rangle\right)\\
%	&+\frac{1}{4}\left(\langle \hat{F}_{[-1,1]}, \hat{F}_{[1,1]} \rangle - \langle \hat{F}_{[-1,1]}, \hat{F}_{[1,\varepsilon]} \rangle + \langle \hat{F}_{[-1,1]}, \hat{F}_{[-1,1]} \rangle - \langle \hat{F}_{[-1,1]}, \hat{F}_{[-1,\varepsilon]} \rangle\right)\\
%	&+\frac{1}{4}\left(-\langle \hat{F}_{[-1,\varepsilon]}, \hat{F}_{[1,1]} \rangle + \langle \hat{F}_{[-1,\varepsilon]}, \hat{F}_{[1,\varepsilon]} \rangle - \langle \hat{F}_{[-1,\varepsilon]}, \hat{F}_{[-1,1]} \rangle + \langle \hat{F}_{[-1,\varepsilon]}, \hat{F}_{[-1,\varepsilon]} \rangle \right)\\
%	& = \frac{1}{4}\left(4 - 4\langle \hat{F}_{[1,1]}, \hat{F}_{[1,\varepsilon]} \rangle + 4\langle \hat{F}_{[1,1]}, \hat{F}_{[-1,1]} \rangle - 4\langle \hat{F}_{[1,1]}, \hat{F}_{[-1,\varepsilon]} \rangle \right)\\
%	&= 1 +  \langle \hat{F}_{[1,1]}, \hat{F}_{[-1,1]} \rangle - \langle \hat{F}_{[1,1]}, \hat{F}_{[-1,\varepsilon]} \rangle\\
%	&= 1 +  \langle \hat{K}_{[1,1]}, \hat{K}_{[1,1]} \rangle  - 1 - \langle \hat{F}_{[1,1]}, \hat{F}_{[-1,\varepsilon]} \rangle - \langle \hat{F}_{[1,1]}, \hat{F}_{[-1,\varepsilon]} \rangle \\
%	& =  \langle \hat{K}_{[1,1]}, \hat{K}_{[1,1]} \rangle - 2\langle \hat{F}_{[1,1]}, \hat{F}_{[-1,\varepsilon]} \rangle\\
%	&= \langle \hat{K}_{[1,1]}, \hat{K}_{[1,1]} \rangle -\frac{1}{2}\left( \langle \hat{K}_{[1,1]}, \hat{K}_{[1,1]} \rangle -  \langle \hat{K}_{[1,\varepsilon]}, \hat{K}_{[1,\varepsilon]} \rangle -\langle \hat{K}_{[-1,1]}, \hat{K}_{[-1,1]} \rangle + \langle \hat{K}_{[-1,\varepsilon]}, \hat{K}_{[-1,\varepsilon]} \rangle \right)\\
%	&= 	\langle \hat{K}_{[1,1]}, \hat{K}_{[1,1]} \rangle -\frac{1}{2}\left( \langle \hat{K}_{[1,1]}, \hat{K}_{[1,1]} \rangle -  \left(2-\langle \hat{K}_{[1,1]}, \hat{K}_{[1,1]} \rangle \right) -\langle \hat{K}_{[-1,1]}, \hat{K}_{[-1,1]} \rangle + \left(2-\langle \hat{K}_{[-1,1]}, \hat{K}_{[-1,1]} \rangle \right) \right)\\
%	&= \langle \hat{K}_{[1,1]}, \hat{K}_{[1,1]} \rangle -\frac{1}{2}\left( 2\langle \hat{K}_{[1,1]}, \hat{K}_{[1,1]} \rangle -  2 -2\langle \hat{K}_{[-1,1]}, \hat{K}_{[-1,1]} \rangle + 2 \right)\\
%%	&= 1 -\langle \hat{K}_{[1,1]}, \hat{K}_{[1,1]} \rangle - \langle \hat{K}_{[1,\varepsilon]}, \hat{K}_{[1,\varepsilon]} \rangle +3\langle \hat{K}_{[-1,1]}, \hat{K}_{[-1,1]} \rangle - \langle \hat{K}_{[-1,\varepsilon]}, \hat{K}_{[-1,\varepsilon]} \rangle\\
%%	& = -1 + 3\langle \hat{K}_{[-1,1]}, \hat{K}_{[-1,1]} \rangle - \langle \hat{K}_{[-1,\varepsilon]}, \hat{K}_{[-1,\varepsilon]} \rangle.
%\end{align*}
%
%Consequently, we obtain \begin{align*}
%1 &= 2\langle \hat{K}_{[-1,1]}, \hat{K}_{[-1,1]} \rangle - \langle \hat{K}_{[-1,\varepsilon]}, \hat{K}_{[-1,\varepsilon]} \rangle\\
%& = 2\langle \hat{K}_{[-1,1]}, \hat{K}_{[-1,1]} \rangle - \left(2- \langle \hat{K}_{[-1,1]}, \hat{K}_{[-1,1]} \rangle\right),
%\end{align*} 
%and thus $$
%  \langle \hat{K}_{[-1,1]}, \hat{K}_{[-1,1]} \rangle = \\
%  \langle \hat{K}_{[-1,\varepsilon]}, \hat{K}_{[-1,\varepsilon]} \rangle = 1.$$
\begin{align*}
	% [ ReflectionSubgroup(CoxeterGroup("E",8), [ 1, 3, 4, 5, 6, 7, 8, 112 ]), 3, 
	%4, CoxeterGroup() ], \\
	%[ ReflectionSubgroup(CoxeterGroup("E",8), [ 1, 2, 3, 5, 6, 7, 8, 116 ]), 6, 
	%12, CoxeterGroup() ], \\
	%[ ReflectionSubgroup(CoxeterGroup("E",8), [ 1, 2, 3, 4, 5, 6, 8, 119 ]), 3, 
	%49, CoxeterGroup("A",1) ] 
\end{align*}



==> e6a3_a1_char_sheaves.tex <==
The preimages that gives $E_6(a_3) +A_1$ 3-special are (keeping Gap3's notations):\\

\[[ ReflectionSubgroup(CoxeterGroup("E",8), [ 1, 3, 4, 5, 6, 7, 8, 112 ]), 3, 
4, CoxeterGroup() ],\]ie. $s = \langle 0,1/3,0,0,0,0,0,0\rangle$, which has a centraliser of type $A_8$, adjoint and $v$ is the unipotent class $222111$
and  \[[ ReflectionSubgroup(CoxeterGroup("E",8), [ 1, 2, 3, 4, 5, 6, 8, 119 ]), 3, 49, CoxeterGroup("A",1) ],\]ie. $s = \langle 0,0,0,0,0,0,1/3,0\rangle$, which has a centraliser of type $E_6 \times A_2$, adjoint and $v$ is the unipotent class $UnipotentClass(A2,111)$.\\

\begin{res}
Using the same reasonning as in \cite{brunatUnitriangularShapeDecomposition2020}. %The Bala-Carter of $E_6(a_3) +A_1$ is $[200202.2]$
and $J = 0,1,2,5,6,7,8$
et $\sigma = w_{\alpha_1}(1/2)$ we obtain that $A = \langle \sigma \rangle$ with a certain $\lambda$ is an admissible covering and $A$ is isomorphic to $A_\G(u)$. 
 
\end{res}

So we need to look at character sheaves with unipotent support $E_6(a_3) + A_1$ and coming from the series $s = \langle 0,0,0,0,0,0,1/3,0\rangle$ and their value at $E_6(a_3) +A_1$ and at $\sigma E_6(a_3) +A_1$.
There are four of them since $\Omega_{C_{\G^*}(s)}(UnipotentClass(A2,111)) \cong S_2$. 
In $W_2 = \Omega_{C_{\G^*}(s)}(UnipotentClass(A2,111))$, the character sheaves with unipotent support $UnipotentClass(A2,111)$ are in the 46th family Family("C2,C1",[46,28,22,79]), they are "phi{30,15},111", "phi{15,16},111", "phi{15,17},111", "D4,:111,111", \\
of which 3 in the principal series
 "phi{30,15},111" -> (2,UnipotentClass(A2,111)), "phi{15,17},111" -> (11,UnipotentClass(A2,111)), "phi{15,16},111" -> (1,UnipotentClass(3A1,111)
 )
 et one induced from a cuspidal pair with Levi of type $D_4$. 

==> e8b6.tex <==
 \subsubsection{The special unipotent conjugacy class $\Cc = E_8(b_6)$ when $\ell = 3$}
 We consider the $F$-stable special unipotent class $\Cc = E_8(b_6)$ when $\ell = 3$. 
 In this case, $A \cong \Omega_{\G,\Cc} \cong S_2$, but $A_\G(u_\Cc)\cong \Omega^3_{\G,\Cc} \cong S_3$ and the class is $\ell$-$P$-special. \\
 We denote the elements of $\Mm(A)$ by $[1,1], [1,\varepsilon], [-1,1],[-1,\varepsilon]$, where $\epsilon$ designs the sign character. 
 
 Thanks to Proposition \ref{excellent} and since $\ell$ does not divide $A$, we can find four unipotent characters $\rho_{[1,1]},\rho_{[1,\varepsilon]},\rho_{[-1,1]},\rho_{[-1,\varepsilon]}$ with unipotent support $\Cc$, and construct four Kawanaka characters with respect to $A$ and $\Cc$ such that \[\langle \rho^*_{[b,\phi]}, K^G_{[a,\psi]} \rangle = \begin{cases} 1 \quad b = a \text{ and } \phi = \psi ,\\
 0 \quad \text{otherwise}.\\

 \end{cases}\]
 However we need $|\mathcal{M}^l(\Omega^3_{\G,\Cc})| = 5$. We need to find an irreducible character of $\G^F$ in the unipotent $\ell$-blocks, which has unipotent support $\Cc$ but isn't unipotent. % It is a problem, because this way we use up all the unipotent irreducible characters with unipotent support $\Cc$...
 
%One possibility: we use other irreducible characters with another unipotent support. Maybe from the unique unipotent conjugacy class not $l$-special ($A_5 + A_1$) and to which we could apply Results \ref{avtgenial} with $A_G(u)$ trivial? Then we will order the unipotent conjugacy classes in the usual order and it should work?  
%
%One possibility: we use other preimages by Lusztig's map. The preimages that gives $E_8(b_6)$ 3-special are (keeping Gap3's notations):\\
%
% \[[ ReflectionSubgroup(CoxeterGroup("E",8), [ 1, 3, 4, 5, 6, 7, 8, 112 ]), 3, 
%11, CoxeterGroup() ],\]ie. $s = \langle 0,1/3,0,0,0,0,0,0\rangle$, which has a centraliser of type $A_8$, adjoint and $v$ is the unipotent class $3321$
%and  \[[ ReflectionSubgroup(CoxeterGroup("E",8), [ 1, 2, 3, 4, 5, 6, 8, 119 ]), 3, 28, CoxeterGroup("A",2) ],\]ie. $s = \langle 0,0,0,0,0,0,1/3,0\rangle$, which has a centraliser of type $E_6 \times A_2$, adjoint and $v$ is the unipotent class $D_{4,111}$.\\

Since $A_\G(u_\Cc)$ is $F$-stable, there are $3$ representatives of $\G^F$ conjugacy classes in $\Cc$, say $u_1$, $u_2$ and $u_3$. 
As in \cite[Proof of Prop. 4.3]{geckUnipotentSupportCharacter2008a}, we have for any unipotent character $\rho$ with unipotent support $\Cc$, \begin{align}\label{eq2}
\sum^{3}_{i =1} [A_\G(u_i) : A_\G(u_i)^F]\langle \rho^*, \Gamma_{u_i}\rangle = \frac{|A_\G(u)|}{n_\rho},
\end{align}

where $n_\rho$ is given by \cite[4.26.3]{lusztigCharactersReductiveGroups1984}. In particular, when $\rho$ is unipotent \[n^{-1}_\rho = 1/2,\] as $\Omega_{\G,\Cc} \cong S_2$. Moreover, as in \cite[Exemple 2.7.8 c)]{geckCharacterTheoryFinite2020}, we may assume that $u_1 $ corresponds to $1$ (whence $[A_\G(u_1) : A_\G(u_1)^F] = 1$), $u_2$ corresponds to a $2$-cycle (whence $[A_\G(u_2) : A_\G(u_2)^F] = 3$), and $u_3$ to a $3$-cycle (whence $[A_\G(u_3) : A_\G(u_3)^F] =2$).\\


Let $\phi \in \irr(S_2)$ and $i,j \in \{\pm 1\}$. By \ref{KawGGGr}, we have that there are two distinct GGGC, say $\Gamma_{v_1}$ and $\Gamma_{v_{-1}}$ 
\begin{align*}
\langle \rho^*_{[i,\phi]},\Gamma_{v_j}\rangle = \delta_{i,j}.
\end{align*}

By construction, we have $\Gamma_{v_1} = \Gamma_{u_1}$ and $\Gamma_{v_{-1}} = \Gamma_{u_2}$. Applying to \ref{eq2}, we must have \[\langle \rho^*_{[1,\phi]},\Gamma_{u_3}\rangle = 1 \text{ and } \langle \rho^*_{[-1,\phi]},\Gamma_{u_3}\rangle = 0.\]

Since $\Cc$ is $\ell$-$P$-special, there $g =sv=vs \in (\G^*)^{F^*}$ with $s (\G^*)^{F^*}$ semisimple of order a power of $3$, and $v \in (\G^*)^{F^*}$ unipotent such that $\Omega_{C_{\textbf{G}^*}(s), v} \cong S_3$ and with $\Phi(g) = \Cc$. . 
%Since the center is connected, by the Jordan decomposition of characters, we can index the characters of $\mathcal{E}(\G,s)_g$ by pairs $[a,\phi] \in \Mm(\Omega_{C_{\textbf{G}^*}(s), v})$.
Now by \cite[Prop. 6.7]{geckCharacterSheavesGeneralized1999} and \cite[Prop 6.7]{hezardSupportUnipotentFaisceauxcaracteres2004}, there is a character $\mu \in \mathcal{E}(\G,s)_g$ such that 
\[\langle \mu^*, \Gamma_{u_i} \rangle = \delta_{3i}.\]

We then choose the irreducible characters $\{\mu, \rho_{[1,1]},\rho_{[1,\varepsilon]},\rho_{[-1,1]},\rho_{[-1,\varepsilon]}\}$ and the projective characters  of $\Oo\G^F$ $\{\Gamma_{u_3},K^\G_{[1,1]},K^\G_{[1,\varepsilon]},K^\G_{[-1,1]},K^\G_{[-1,\varepsilon]}\}.$

We can check that the decomposition matrix of $\G^F$ restricted to these rows of irreducible characters and columns of projective characters of is unitriangular. In fact it even has the shape of the identity matrix.


%We now distinguish between $6$ different cases and observe how it applies to (\ref{eq1}):
%\begin{enumerate}
%\item when $\Gamma_{v_1} = \Gamma_{u_1}$ and $\Gamma_{v_{-1}} = \Gamma_{u_2}$, then for $\phi \in \irr(S_2)$, we must have \[\langle \rho^*_{[1,\phi]},\Gamma_{u_3}\rangle = 1 \text{ and } \langle \rho^*_{[-1,\phi]},\Gamma_{u_3}\rangle = 0.\]
%\item when $\Gamma_{v_1} = \Gamma_{u_1}$ and $\Gamma_{v_{-1}} = \Gamma_{u_3}$, then for $\phi \in \irr(S_2)$, is not possible because then \[3 = \sum_{3}^{i =1} [A_\G(u_i) : A_\G(u_i)^F]\langle \rho^*_{[1,\phi]}, \Gamma_{u_i}\rangle = 1 + 3\langle \rho^*_{[1,\phi]}, \Gamma_{u_2}\rangle. \]
%\item when $\Gamma_{v_1} = \Gamma_{u_2}$ and $\Gamma_{v_{-1}} = \Gamma_{u_1}$, then for $\phi \in \irr(S_2)$, we must have \[\langle \rho^*_{[1,\phi]},\Gamma_{u_3}\rangle = 0 \text{ and } \langle \rho^*_{[-1,\phi]},\Gamma_{u_3}\rangle = 1.\]
%\item when $\Gamma_{v_1} = \Gamma_{u_2}$ and $\Gamma_{v_{-1}} = \Gamma_{u_3}$, then for $\phi \in \irr(S_2)$, we must have \[\langle \rho^*_{[1,\phi]},\Gamma_{u_1}\rangle = 0 \text{ and } \langle \rho^*_{[-1,\phi]},\Gamma_{u_1}\rangle = 1.\]
%\item when $\Gamma_{v_1} = \Gamma_{u_3}$ and $\Gamma_{v_{-1}} = \Gamma_{u_1}$, then for $\phi \in \irr(S_2)$, is not possible because then \[3 = \sum_{3}^{i =1} [A_\G(u_i) : A_\G(u_i)^F]\langle \rho^*_{[-1,\phi]}, \Gamma_{u_i}\rangle = 1 + 3\langle \rho^*_{[-1,\phi]}, \Gamma_{u_2}\rangle. \]
%\item when $\Gamma_{v_1} = \Gamma_{u_3}$ and $\Gamma_{v_{-1}} = \Gamma_{u_2}$, then for $\phi \in \irr(S_2)$, we must have \[\langle \rho^*_{[1,\phi]},\Gamma_{u_1}\rangle = 1 \text{ and } \langle \rho^*_{[-1,\phi]},\Gamma_{u_1}\rangle = 0.\]
%\end{enumerate}
%
%Let us now consider irreducible characters $\mu \in \mathcal{E}(\G,s)_g$ with $g =sv$ such that $\Omega_{C_{\textbf{G}^*}(s), v} \cong S_3$ and with $\Phi(g) = \Cc$. We know it exists such a $g$ with $s$ a $3$-element. 
%Since the center is connected, by Jordan decomposition of characters, we can index the characters of $\mathcal{E}(\G,s)_g$ by pairs $[a,\phi] \in \Mm(\Omega_{C_{\textbf{G}^*}(s), v})$.
%
%Again as in \cite[Proof of Prop. 4.3]{geckmeinolfUnipotentSupportCharacter2008}, we have for any character $\mu \in \mathcal{E}(\G,s)_g$ with unipotent support $\Cc$, \begin{align}\label{eq2}
%\sum_{3}^{i =1} [A_\G(u_i) : A_\G(u_i)^F]\langle \mu^*, \Gamma_{u_i}\rangle = \frac{|A_\G(u)|}{n_\rho},
%\end{align}
%where $n_\rho $ is given by \cite[4.26.3]{lusztigCharactersReductiveGroups1984}. 
%When $\mu = \mu_{[1,1]}$, then we have $n_\rho = |S_3|$. Thus, \[\langle \mu^*_{[1,1]}, \Gamma_{u_i}\rangle = \delta_{1,i}.\]
%Assume that $\mu = \mu_{[1,\text{ref}]}$, where $\text{ref} \in \irr(S_3)$ is the unique irreducible character of degree $2$.We then have $n^{-1}_\rho = 2/|S_3|$. Thus, \[\langle \mu^*_{[1,\text{ref}]}, \Gamma_{u_i}\rangle = \delta_{3,i}.\]
%
%We then choose \begin{itemize}
%	\item in cases 1. and 3. the irreducible characters $\{\mu_{[1,\text{ref}]}, \rho_{[1,1]},\rho_{[1,\varepsilon]},\rho_{[-1,1]},\rho_{[-1,\varepsilon]}\}$ and the projective characters $\{\Gamma_{u_3},K^\G_{[1,1]},K^\G_{[1,\varepsilon]},K^\G_{[-1,1]},K^\G_{[-1,\varepsilon]}\}$, 
%	\item and in cases 4. and 6. the irreducible characters $\{\mu_{[1,1]}, \rho_{[1,1]},\rho_{[1,\varepsilon]},\rho_{[-1,1]},\rho_{[-1,\varepsilon]}\}$ and the projective characters $\{\Gamma_{u_1},K^\G_{[1,1]},K^\G_{[1,\varepsilon]},K^\G_{[-1,1]},K^\G_{[-1,\varepsilon]}\}$.
%\end{itemize}
%
%We can check that the decomposition matrix of $\G^F$ restricted to these rows of irreducible characters and columns of projective characters is unitriangular. 
